Reversible Action Design for Combinatorial Optimization with Reinforcement Learning

Combinatorial optimization problem (COP) over graphs is a fundamental challenge in optimization. Reinforcement learning (RL) has recently emerged as a new framework to tackle these problems and has demonstrated promising results. However, most RL solutions employ a greedy manner to construct the solution incrementally, thus inevitably pose unnecessary dependency on action sequences and need a lot of problem-specific designs. We propose a general RL framework that not only exhibits state-of-the-art empirical performance but also generalizes to a variety class of COPs. Specifically, we define state as a solution to a problem instance and action as a perturbation to this solution. We utilize graph neural networks (GNN) to extract latent representations for given problem instances for state-action encoding, and then apply deep Q-learning to obtain a policy that gradually refines the solution by flipping or swapping vertex labels. Experiments are conducted on Maximum $k$-Cut and Traveling Salesman Problem and performance improvement is achieved against a set of learning-based and heuristic baselines.

==> NeurIPS2020/abstract.tex <==
 \begin{abstract}
Combinatorial optimization problem (COP) over graphs is a fundamental challenge in optimization. Reinforcement learning (RL) has recently emerged as a new framework to tackle these problems and has demonstrated promising results. However, most RL solutions employ a greedy manner to construct the solution incrementally, thus inevitably pose unnecessary dependency on action sequences and need a lot of problem-specific designs. We propose a general RL framework that not only exhibits state-of-the-art empirical performance but also generalizes to a variety class of COPs. Specifically, we define state as a solution to a problem instance and action as a perturbation to this solution. 
We utilize graph neural networks (GNN) to extract latent representations for given problem instances for state-action encoding, and then apply deep Q-learning to obtain a policy that gradually refines the solution by flipping or swapping vertex labels. 
%A auxiliary action-proposal network is also applied to cope with the potential large action space. 
%With this local search manner, our method improves the quality of solutions by enabling the agent to jump out of the local minima and provides extra flexibility when dealing with different COPs. 
Experiments are conducted on Maximum $k$-Cut and Traveling Salesman Problem and performance improvement is achieved against a set of learning-based and heuristic baselines.

\end{abstract}

==> NeurIPS2020/conclusion.tex <==
\section{Conclusions and Future Work}
In this paper, we introduced a general end-to-end RL framework for solving combinatorial optimization problems on graphs. 
The key idea behind our design is to view a solution to a problem instance as state and reversible perturbation to this solution as action. We introduce graph neural networks to extract latent representations of graphs for state-action encoding, and  apply deep Q-learning to obtain a policy that gradually improves the solution.
%The key idea behind our design is the reversible action that allows the agent to constantly improve the solution starting from an arbitrary one. We believe the flipping and swapping action space we proposed can be applied to many COPs, as any two elements in their solution space can be connected through a sequence of these two types of actions. 
We instantiated the meta-algorithm for Maximum $k$-Cut and TSP, where extensive experiment results demonstrate the solution's competitive performance and generalization across problem instances. 
%As we have shown in the experiments, greedy algorithms that take the flipping and swapping actions are already very strong baselines, and RL training can further lift the agent to take more informed actions rather than greedy moves.
%Like most previous RL-based solutions for COPs, our framework also demonstrates a good generalization ability to larger test instances.
One obstacle that prevents its application to large graphs is the formidable size of swapping action space, which has been successfully addressed by introducing an auxiliary action-proposal network. 
%We believe that our work could shed some light on the algorithm design for the combinatorial optimization community. 

One important direction of this work is the refinement of the state representation. 
%Our current design does not fully consider the combinatorial structure of the solution: we use one-hot labels on vertices to represent a graph cut and a sequence to represent a tour in TSP. Although they work well empirically, 
The permutation/rotation invariant issue raises some concern: solutions that are equivalent under a permutation or rotation of vertex labels will lead to a totally different representation. This costs an unnecessarily large input space and burden on the capacity of the neural network. Several existing works also mentioned this issue \cite{zaheer2017deep,rezatofighi2018deep,meltzer2019pinet,wagstaff2019limitations}, but did not provide an effective solution yet.
%they mainly focused on the representation of sets, which is not sophisticated enough for most combinatorial problems: in the case of Maximum $k$-Cut, the solution is a nested set and in TSP the solution is a cycle). 
To design a network architecture that encodes various nontrivial combinatorial structures remains a challenging yet promising direction.


\section{Broader Impact}
Many real-world problems, such as vehicle routing \cite{dantzig1959truck}, resource allocation \cite{han2008resource}, and logical analysis for medical systems \cite{hammer2006logical}, boil down to combinatorial optimization problems. Our framework offers a learning-based solution to improve optimality for this family of problems, which are typically addressed by heuristics. The generalization ability of our RL solution enables it to scale to problems of various sizes and involves less ad-hoc designs or domain-knowledge. 

A potential drawback of our solution lies in its explainability, i.e., why a certain action is taken by the agent can hardly be interpreted. Especially under the circumstances where the immediate reward of the chosen actions might be negative, e.g., the agent is trying to jump out of local minima. This might cause undesirable issues in important decision-making scenarios, such as resource allocation in economy and medical data analysis. The current efforts in explainable machine learning should be a good direction to improve this potential limitation. 

==> NeurIPS2020/exp.tex <==
\section{Experiments}
\subsection{Problem Setups}
We evaluate our proposed solution framework on Maximum $k$-Cut and TSP. For Maximum $k$-Cut, we consider two settings: Maximum Cut (i.e., $k$=2) and Maximum $k$-Cut with size constraint (i.e., $k>2$ and the sizes of the graph cut are given). For the training, validation and test set of Maximum Cut, we use complete graphs whose weighted adjacency matrices are given by the pairwise Euclidean distances among $n$ nodes uniformly sampled from $[0, 1]^h$. For Maximum $k$-Cut, we use a synthetic dataset generated by $k$-clustered graph, where each problem instance $G=(V, E, w)$ is a complete graph generated by first sampling $k$ centroids $\{c_1, \cdots, c_k\}$ uniformly from $[0, 1]^h$, and then sample $m$ nodes $\{x_{ij}\}_{j=1}^{m}$ for each centroid $c_i$ from Gaussian distribution $N(c_i, \sigma^2_i I_h)$, where $m, h, \sigma_i$ are hyper-parameters and $I_h$ is the identity matrix of size $h$. The weighted adjacency matrix $w$ is then computed as the Euclidean distances between each pair of nodes, i.e., $w_{ij}=||x_i-x_j||_2$. For TSP, we draw training graphs from a distribution where each node $x_i$ is uniformly sampled from a 2-D square $\{(x, y)| 0\leq x \leq 1, 0\leq y \leq 1\}$ and the weighted adjacency matrix $w$ is computed by Euclidean distances accordingly, i.e., $w_{ij}=||x_i-x_j||_2$. For the testing set of TSP, we resort to a public benchmark TSPLIB derived from real-world instances \cite{TSPLIB}. 

Note that in our settings all training and validation graphs are complete graphs, which is computationally cumbersome when $n$ becomes large. To scale up for larger $n$ (e.g., $n>50$), we use the $K$-nearest neighbor graph ($K = 50$) to replace the complete graph, i.e., reserve top-$K$ nearest neighbors in the weighted adjacency matrix.    

\subsection{Metrics and baselines}

For Maximum Cut, we consider two RL-based baselines S2V-DQN \cite{khalil2017learning} and ECO-DQN \cite{ecodqn}. In addition, we consider several popular heuristic-based methods including semidefinite programming (SDP) \cite{sdp}, genetic programming (GP) \cite{gp}, and greedy algorithm. SDP is a non-greedy algorithm that gives a solution by relaxing the discrete problem to a continuous one and then applying semidefinite programming to address the resulting optimization problem. GP is an evolutionary computation method that imitates biological evolution by iteratively improving a set of solutions through mutations and selections. The greedy algorithm we use here is an iterative method that starts with a random cut and flips or swaps the label of a vertex at each step with the greatest immediate increase in the cut value until no further improvement can be made, which corresponds to a RL agent in our framework that always follows the one-step reward.  

For Maximum $k$-Cut ($k$>2) with size constraint, S2V-DQN and ECO-DQN cannot directly apply. As a result, we use three heuristic baselines, i.e., SDP, GP, greedy algorithm for benchmarking. Note that the greedy algorithm we use here takes swapping as an action to guarantee the size constraints. 

For the baselines of TSP, we include S2V-DQN and two approximation algorithms Farthest insertion (Farthest) and 2-opt, which are reported as the two best-performing approximation methods on TSPLIB dataset \cite{khalil2017learning}. The implementation details for these two approximation algorithms can be found in \cite{applegate2006traveling}. Note that the 2-opt method is essentially the greedy algorithm that takes the swapping action as we designed for TSP.

We use the approximation ratio $R^{app}=O^*/O^{opt}$ as a metric to evaluate the quality of solutions, where $O^*$ is the best objective value given by an algorithm, and $O^{opt}$ is the true optimal objective value. For Maximum $k$-Cut problems with large sizes, we do not have access to $O^{opt}$. Considering that the greedy algorithm demonstrates itself as the strongest baseline for large-scale Maximum $k$-Cut problems, we apply it multiple times with different initial solutions and take its best result as the alternative for $O^{opt}$. For the test problem instances of TSP, $O^{opt}$ is provided in the TSPLIB dataset.

\subsection{Solution quality comparison}

To compare the quality of solutions, we train our algorithm with problem instances up to 200 nodes and test it on 100 held-out graphs of the same size. The maximum episode length is set to twice the size of the graph; and during each training epoch, the training batch is sampled uniformly from $\mathcal{D}$ with a randomly initialized solution, with the batch sizes ranging from 50 to 500 to meet the memory limitation posed by a single graphic card. The agent starts planning from a randomly initialized solution on each test instance. Table \ref{tab:kcut} and \ref{tab:tsp} summarize the results on the average approximation ratio across Maximum Cut, Maximum $k$-Cut, and TSP with variance over multiple trials (i.e. different trials are the trajectories starting from randomly drawn initial states) shown on the superscripts and subscripts. Our algorithm is denoted by the name LS-DQN (i.e. Local Search DQN). 

For Maximum Cut with $k=2$, the flipping action design is employed in our solution. As shown in Table \ref{tab:kcut}, LS-DQN performed as good as ECO-DQN and outperformed S2V-DQN on larger test graphs. Compared to approximation heuristics such as SDP and GP, LS-DQN showed a better and more stable performance, and the gain became more significant as the test graph size increases. It is not a surprise to observe the greedy baseline has strong performance, because it can always guarantee a local minimum (i.e., there is no flipping that generates immediate improvement); and in Maximum Cut, local minima were close to the global minimum with very high probability based on our observations. The performance gain of LS-DQN mainly comes from its ability to jump out of those local minima during planning. For Maximum $k$-Cut, we test our model on three different graph scales: $(k, m)=(5,6), (10,10), (10,20)$. As shown in the bottom of Table \ref{tab:kcut}, LS-DQN performed significantly better than SDP and GP, and slightly better than the greedy algorithm. Table \ref{tab:tsp} shows the result for TSP. The Farthest and 2-opt algorithms are the two strongest baselines for the TSPLIB dataset according to the results reported in \cite{khalil2017learning}. As the graph sizes in TSPLIB are not identical to our training size, we train our RL agent on graphs with fixed sizes and test it on-the-fly on a batch of graphs whose sizes fall in a certain range, and report the result on the best tour encountered over the training epochs, like it was done in \cite{khalil2017learning}. Our LS-DQN reaches the best approximation ratio on graph sizes up to 200 compared to S2V-DQN and the other two heuristics. 

\begin{table}[t]
\centering
\caption{\label{tab:kcut}Approximation ratio comparison for Maximum $k$-Cut ($k=2$). Larger is better.}
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Train/Test Size & LS-DQN & S2V-DQN & ECO-DQN & SDP & GP & Greedy \\\hline
$n=20$ & $0.98^{+0.02}_{-0.02}$& $0.98^{+0.01}_{-0.01}$& $0.99^{+0.01}_{-0.02}$& $0.98$& $0.96^{+0.03}_{-0.03}$& $0.98^{+0.02}_{-0.02}$\\\hline
$n=50$ & $0.98^{+0.02}_{-0.02}$& $0.97^{+0.02}_{-0.02}$& $0.98^{+0.02}_{-0.02}$& $0.97$& $0.96^{+0.03}_{-0.03}$& $0.97^{+0.02}_{-0.02}$\\\hline
$n=100$ & $0.97^{+0.01}_{-0.01}$& $0.94^{+0.02}_{-0.02}$& $0.97^{+0.02}_{-0.02}$& $0.95$& $0.92^{+0.03}_{-0.03}$& $0.94^{+0.02}_{-0.02}$\\\hline
$n=200$ & $0.95^{+0.01}_{-0.01}$& $0.94^{+0.02}_{-0.02}$& $0.96^{+0.01}_{-0.01}$& $0.89$& $0.85^{+0.02}_{-0.02}$& $0.93^{+0.02}_{-0.02}$\\\hline
$(k, m)=(5, 6)$& $0.98^{+0.02}_{-0.02}$& -&-&  $0.92$& $0.67^{+0.05}_{-0.05}$& $0.98^{+0.02}_{-0.02}$\\\hline
$(k, m)=(10, 10)$& $0.97^{+0.02}_{-0.02}$& -&-& $0.89$& $0.42^{+0.05}_{-0.05}$& $0.96^{+0.02}_{-0.02}$\\\hline
$(k, m)=(10, 20)$& $0.95^{+0.02}_{-0.02}$& -&-& $0.86$& $0.34^{+0.04}_{-0.04}$& $0.94^{+0.02}_{-0.02}$\\\hline
\end{tabular}
\label{tab:kcut}
\vspace{-3mm}
\end{table}
% \FloatBarrier

\begin{table}[H]
\centering
\caption{\label{tab:tsp}Approximation ratio comparison for TSP. Smaller is better.}
\begin{tabular}{c|c|c|c|c|c}
\hline
Train Size & Test Size & LS-DQN  & S2V-DQN & Farthest & 2-opt \\\hline
$n=50$&51-100& $1.04^{+0.01}_{-0.01}$& $1.05^{+0.01}_{-0.01}$& $1.07^{+0.01}_{-0.01}$& $1.07^{+0.01}_{-0.01}$\\\hline
$n=100$&101-150& $1.05^{+0.01}_{-0.01}$& $1.05^{+0.01}_{-0.01}$& $1.08^{+0.01}_{-0.01}$& $1.09^{+0.01}_{-0.01}$\\\hline
$n=150$&151-200& $1.06^{+0.01}_{-0.01}$& $1.07^{+0.01}_{-0.01}$& $1.08^{+0.01}_{-0.01}$& $1.09^{+0.01}_{-0.01}$\\\hline
\end{tabular}
\label{tab:tsp}
\vspace{-3mm}
\end{table}
% \FloatBarrier

\subsection{Generalization to larger graphs}
To investigate the generalization ability of our solution on both Maximum Cut and TSP, we train our RL agent on small graphs of a fixed size ($n=50$) and test it on larger graphs with sizes up to 300. Table \ref{tab:generalize} summarizes the results with the comparison to S2V-DQN, where the reported values are the approximation ratios averaged over 100 test graphs. As we can see, LS-DQN achieved encouraging and consistent approximation ratios across different test graph sizes on both tasks. LS-DQN generalizes as good as S2V-DQN on Maximum $k$-Cut, and has shown some advantage on TSP tasks. This confirms the generalization of our proposed RL solution framework and the applicability of learned agents across distinct problem instances.

\begin{table}[t]
\caption{Evaluation of generalization of LS-DQN (LS) and comparison with S2V-DQN (S2V). Models are trained on graphs with 50 nodes, and tested on larger sizes up to 300. The average approximation ratio over different testsets is reported.}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline 
Test Size & \multicolumn{2}{c}{51-100} & \multicolumn{2}{|c}{101-150}  & \multicolumn{2}{|c}{151-200} & \multicolumn{2}{|c}{200-300} \\\hline
Algorithm & LS & S2V& LS & S2V& LS & S2V& LS & S2V \\\hline
MAXCUT& 0.984& 0.988& 0.974 &0.971& 0.972 &0.975 & 0.978&0.981\\\hline
TSP& 1.034 &1.075& 1.054& 1.089& 1.088 &1.087& 1.094&1.095\\\hline
\end{tabular}
\normalsize
\label{tab:generalize} 
\vspace{-3mm}
\end{table}
% \FloatBarrier

\subsection{Trade-off between efficiency and accuracy}

As we have discussed in Section \ref{end2end}, the deployment of the action-proposal network (AP-net) is essential to enable our method to scale to large graphs. In the AP-net, the action reserve ratio $\epsilon \in (0, 1]$ controls the proportion of actions being evaluated at each state: a large $\epsilon$ allows the agent to evaluate q-values on more state-action pairs, which enhances the quality of planning but also increases the time and space complexity. We investigate the trade-off between efficiency and approximation ratio in our solution. Figure \ref{fig:tradeoff} shows the training curve for Maximum $k$-Cut and TSP under different action reserve ratios. We choose $\epsilon \in \{1.0, 0.5, 0.01, 0.05, 0.01\}$, and a baseline that randomly samples 10\% actions without using the AP-net. As we can find, the performance gap is nearly negligible when $\epsilon \geq 0.1$. When $\epsilon \leq 0.05$, the performance drop becomes sensible, but the approximation ratio when reserving only 1\% actions proposed by the AP-net is still better than randomly selecting 10\% actions. Table \ref{tab:tradeoff} lists the relative running time and memory cost when applying different $\epsilon$. It shows that we can maintain $99\%$ performance in terms of the approximation ratio while only consuming approximately $10\%$ time and space for Maximum $k$-Cut. For TSP, since we adopt an RNN structure in the Q-net, the time and space savings are acceptable but not as significant as in Maximum $k$-Cut. 

\begin{figure}
\centering
\subfigure[Maximum $k$-Cut]{
\label{fig:subfig:a}
\includegraphics[width=0.40\textwidth]{resource/1_1.pdf}}
\hspace{.2in}
\subfigure[TSP]{
\label{fig:subfig:b}
\includegraphics[width=0.40\textwidth]{resource/1_2.pdf}}
\vspace{-3mm}
% \begin{minipage}[c]{0.3\textwidth}
%     \caption{

%     }
\caption{Learning curves for Maximum $k$-Cut and TSP with different action reserve ratios. The test performance is evaluated every 200 epochs in Maximum $k$-Cut and every 100 epochs in TSP. 
%The best performance is achieved when action elimination is not applied (i.e., A.R. ratio=1.0) while the worse performance comes with randomly cut off $90\%$ actions for q-value evaluation at each state (Random 0.1). The curves indicate the effectiveness of our AP-net: an A.R. ratio around 0.1 does little harm to the performance, and the performance by choosing an A.R. ratio=0.01 can still beat the baseline that randomly reserves $10\%$ actions.
}
\label{fig:tradeoff} %% label for entire figure
\vspace{-3mm}
\end{figure}

\begin{table}[H]
\caption{\label{tab:tradeoff kcut}Trade-off between time/space complexity and the Approx. ratio (A.R.) with different action reserve ratios $\epsilon$ in the AP-net. The value shown in the table is scaled according to the result at $\epsilon=1.0$. %For the approximation ratio, the larger the better; for the time and space costs, the lower the better.
}
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
$\epsilon$  & \multicolumn{3}{c}{0.5} & \multicolumn{3}{|c}{0.1} & \multicolumn{3}{|c}{0.05} & \multicolumn{3}{|c}{0.01} \\\hline
&  A.R. & Time & Space & A.R. & Time & Space & A.R. & Time & Space & A.R. & Time & Space  \\\hline
$k$-Cut&  1.00& 0.51 & 0.53& 0.99& 0.11&0.14& 0.95&0.06&0.10& 0.82 &0.02&0.06\\\hline
TSP&  1.00 & 0.68&0.51& 0.98&0.29&0.12& 0.93&0.23&0.09& 0.80 &0.19&0.06\\\hline
\end{tabular}
\normalsize
\label{tab:tradeoff}
\vspace{-3mm}
\end{table}


% \begin{table}
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% \hline
% Instance & OPT & LS-DQN & S2V-DQN & 2-opt & Farthest \\\hline
% eil51 & 426 &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\
%  &  &  &  &  &  \\\hline
% \end{tabular}
% \caption{\label{tab:tradeoff kcut}TSPLIB results}
% \end{table}




==> NeurIPS2020/intro.tex <==
\section{Introduction}

Combinatorial optimization problems (COP) have attracted extensive interest from both machine learning and operation research communities in decades because of its pervasive application scenarios \cite{grotschel1991optimal, plante1987product, waldspurger2015phase, candes2015phase}. Most of these problems are known to be NP-hard \cite{karp1972reducibility} and extremely challenging for their combinatorial nature: the optimization is performed over a discrete structure (e.g. a weighted graph) and is often associated with exponentially sized feasible solution space. To give a concrete example, consider Maximum $k$-Cut: given a weighted graph $G=(V, E)$, find a partition of $V$ that divides $G$ into $k$ disjoint sets which maximize the sum of edge weights among each pair of partitions. Another popular example is Traveling Salesman Problem (TSP), in which the goal is to search for the shortest possible route that visits each node on a graph once and only once and returns to the origin node. 

Since the solution domain of COP is prohibitively large, exact methods, such as enumeration based approaches are simply intractable. Therefore, classical solutions for COPs mainly focused on heuristics for decades; such methods include simulated annealing \cite{patel1991preliminary} and genetic algorithms \cite{dedieu2003design}.
%, which all have proven to be acceptable in many practical applications \cite{sorensen2013metaheuristics}.
However, these heuristics often suffer from arduous case-specific design and redundant computation because common combinatorial structures have to be addressed repeatedly across similar problem instances. Recently, learning-based methods have emerged as an effective tool to provide generalizability across similar problems by exploiting the structure of the target problem. In particular, reinforcement learning (RL) has been identified as a powerful end-to-end framework \cite{bello2016neural, ma2019combinatorial,kool2018attention,abe2019solving,ecodqn}, because it does not rely on ground-truth solutions compared to supervised methods \cite{vinyals2015pointer, li2018combinatorial, mittal2019learning, nowak2017note, joshi2019efficient}. However, most RL-based attempts are tailored for a single class of COPs and require a lot of domain-specific designs. For instance, \citet{bello2016neural} adopt the Pointer Network structure \cite{vinyals2015pointer} to encode a permutation of vertex set for TSP, but it is specifically designed to tackle COPs for which the output depends on the length of the input. \citet{ma2019combinatorial} resort to a hierarchical RL structure to address TSP with time-window constraints, but such design is only tailored for TSP and can hardly generalize to other COPs. To alleviate the issue, \citet{khalil2017learning} proposed a general framework, S2V-DQN, to cope with a wide range of COPs by combining graph neural network (GNN) and deep Q-learning. However, S2V-DQN's node selection strategy is greedy in nature, which prevents it from yielding high-quality solutions since the learned policy cannot revoke its previous decisions based on the observations afterward. Moreover, this greedy node selection strategy suffers when the target COPs have non-sequential structured solutions, e.g., Maximum $k$-Cut with $k>2$, because a sequence of irreversible node selections is not an effective way to form graph partitions. 

We propose a new general RL framework for COPs with reversible action design. Similar to S2V-DQN, our method also consists of a GNN encoder for state-action encoding and a deep Q-network for policy learning. However, unlike S2V-DQN and other similar approaches in which the agent builds solutions with irreversible actions, our formulation allows RL agents to explore the whole solution space starting from an arbitrary solution and keep improving it. Another strength of our framework is the ability to handle a wider range of COPs with different solution structures. 
%Compared to ECO-DQN \cite{ecodqn}, which only handles Maximum 2-Cut problem, 
Our method precludes any ad-hoc designs in the RL formulation and leaves problem-specific properties to the state-action encoding networks. As a result, it can easily transfer to different COPs by applying different state-action encoders while maintaining all other essential designs in the RL module. We tested our framework on two extensively studied COPs, Maximum $k$-Cut and TSP, on both synthetic and real-world datasets and obtained competitive performance compared to both learning-based methods and heuristic baselines. In addition to the encouraging performance, we also observed that the trained agent has learned to approach the optimal solution with the ability to jump out of the local minima along the way, which is the key bottleneck of greedy or heuristic based solutions.

% In the following sections, we will first introduce the background related to our proposed framework and formalize our method in detail. Then we'll apply our framework on two extensively studied COPs, Maximum $k$-Cut and TSP, and further present experimental results on several synthesized datasets along with the comparison with S2V-DQN, ECO-DQN, and other traditional approaches. Finally, we'll discuss some fundamental challenges that we identified in our experiments. We believe that our work could shed some light on the algorithm design for the combinatorial optimization community. 


==> NeurIPS2020/method.tex <==
\section{Method}
\subsection{Problem Formulation}
%In a nutshell, we formulate the common definition of combinatorial optimization problem (COP) as follows: $S$ is a finite set of elements, $f: S \xrightarrow[]{} \mathbb{R}$ is a cost function, and the aim of a COP is to find the optimal value of $f$ on $S$. Since the domain $S$ is finite, the global optimum always exists. But in most cases, $S$ is formidably large, and therefore trivial enumeration-based solutions are not feasible. In this work, we focus on the COPs where $S$ displays a graph structure. With a slight abuse of terminology, we use COP to denote combinatorial optimization problems on graphs. In this case, we can further specify the essential components of a COP as follows:

In this work, we focus on the COPs where the problem instances impose a weighted graph structure. With a slight abuse of terminology, we use COP to denote combinatorial optimization problems on graphs. In this case, we can specify the essential components of a COP as follows:
\begin{enumerate}[leftmargin=*]
    \item A problem instance, i.e. a weighted graph $G\!=\!(V,\! E,\! w)$ sampled from some underlying distribution $\mathcal{D}$, where $V\!=\!(v_1,\cdots,v_n)$, $E\!=\!(e_1,\cdots,e_m)$ and $w\!=\!\{w(v_i, v_j)\}$ represent the vertex set, the edge set and the weights associated with each edge, respectively. For simplicity, we denote $w_{ij}\!=\!w(v_i, v_j)$ and simply assign $w_{ij}\!=\!0$, if $v_i$ and $v_j$ are not directly connected. In this case, $G$ can be fully expressed by the weighted adjacency matrix $w$.
    \item A solution to a problem instance $G$ given by a mapping $l$ from $V$ to $\mathbb{N}$, which assigns an integer-valued label to each vertex. For simplicity, we denote the solution as $L\!=\!(l(v_1), \cdots, l(v_n))$.
    \item An objective function $O(G, L) \!\in \!\mathbb{R}$ that takes a problem instance $G$ and a solution $L$ as input and outputs the evaluation on $(G, L)$. The goal of a COP is to find a global optimal solution $L^*_G\!=\!\text{argmin}_{L}O(G, L)$ under certain constraints to $L$.
\end{enumerate}
Since the solution space on a finite graph $G$ is also finite, its global optimum $L^*_G$ always exists if the problem is feasible. But in most cases, as the solution space of $l$ is formidably large, trivial enumeration-based solutions are not feasible. 

Given the abstract formulation above, we can instantiate some popular COPs by specifying different $G$, $L$ and $O$. For example, consider Maximum $k$-Cut, where $G$ is an arbitrary weighted graph, $L$ is an element from $\mathcal{L}\!=\!\{(l_1, \cdots, l_n)| l_i \!\in\! \{1, 2, \cdots, k\} \}$, and $O\!=\!\sum_{c=1}^{k}\sum_{(i,j) \in \{i,j|l_i=l_j=c\}}w_{ij}$. Similarly we can formulate TSP as: $G$ is a complete graph characterized by a weighted adjacency matrix $w$, $L$ is an element in the set of all permutations of $\{1,2,\cdots,n\}$, and  $O\!=\!w_{l_1l_n}\!+\!\sum_{k=1}^{n-1}w_{l_kl_{k+1}}$.
In this paper, we illustrate our solution framework using Maximum $k$-Cut and TSP, because they represent two typical classes of COPs in a broad sense. TSP represents COPs with sequentially structured solutions, such as vehicle routing problem \cite{dantzig1959truck}; and Maximum $k$-Cut represents COPs that fall into the category of node classification, such as Minimum Vertex Cover and Maximal Independent Set. By designing meta-algorithms for solving Maximum $k$-Cut and TSP, we demonstrate how our methodology can shed light on finding solutions for a wide range of related COPs.

\subsection{Reinforcement Learning Solution Design}

We apply reinforcement learning to design a meta-algorithm that minimizes the discrete objective function $O(G, L)$. Unlike the greedy strategy employed by S2V-DQN \cite{khalil2017learning}, in which the agent is trained to construct the solution sequentially by adding nodes to a partial solution, our design allows the agent to gradually improve a given solution $L$ by adding small perturbations to it at each step. Specifically, we define the primitive components in our RL formulation as follows:
\begin{enumerate}[leftmargin=*]
\item State space. The state space $\mathcal{S}\!=\!\{s\!=\!(G, L)|G \in \mathcal{D}, L\in \mathcal{L}_G\}$ ($L$ may depend on $G$) is defined as the set of all the valid graph-solution pairs. Note that the distribution $\mathcal{D}$ might contain graphs with different sizes. 
\item Action space. The action space $\mathcal{A}(s)$ is designed as all valid perturbations on $L$ given a state $s\!=\!(G, L)$, plus a dummy action $\emptyset$ which terminates further actions. $\mathcal{A}(s)$ includes those perturbations such that the perturbed $L$ is still a valid solution in $\mathcal{L}$ for $G$. In particular, we define two types of perturbations on $L$:
\begin{enumerate}
\item  Flipping $\mathcal{A}^{flip}$, in which an action $a$ flips the label $l_i$ for node $v_i$ into a different one.
\item  Swapping $\mathcal{A}^{swap}$, in which an action $a$ swaps the label $l_i$ and $l_j$ for node pair $(v_i, v_j)$.
\end{enumerate}
\item Reward. The reward function $r(s, a)$ is defined as the negative value change for the objective function $O$ after taking action $a$ at state $s\!=\!(G, L)$, i.e., $r(s, a)\! =\! O(G, L) \!- \!O(G, a \circ L)$.
\item Policy. We adopt the Q-learning framework to fit a Q-function $Q(s, a)$ that evaluates the accumulated reward given any state-action pair. According to the learned q-value, we apply a deterministic policy $\pi(s)\!=\!\argmax_{a \in \mathcal{A}(s)} Q(s, a)$.
\item Termination. An episode is terminated when the agent decides to take the dummy action $\emptyset$, or the maximum number of actions $M$ have been executed, where $M$ is a hyper-parameter and grows with the graph size $n$.
\end{enumerate}
Apart from the difference in action design, another distinction between our work and S2V-DQN lies in the construction of states: in S2V-DQN, the state is a graph with a partial solution; while in our framework the state is a graph with a complete solution. As a result, our solution can always exploit the complete structure of a solution at each step, while S2V-DQN struggles with incomplete information to take the next action, especially in the first few steps when the partial solution only consists of a few scattered nodes. Another advantage of our framework is its flexibility when dealing with inherent or additional constraints, e.g., the permutation constraint in TSP (i.e. no duplicated nodes on a route), or the cut-size constraints in Maximum $k$-Cut (i.e. given size of each subgraph induced by the cut). To address these constraints, we only need to pose restrictions on the action space to guarantee that each perturbed solution also satisfies the constraints. But in S2V-DQN and other works, such as \cite{bello2016neural} which also adopts S2V-DQN's greedy design pattern, ad-hoc changes to the architecture of the Q-network have to be made to handle the constraints.

\subsection{State/Action Representation and Q-function Parameterization}
To apply Q-learning for solving COPs, we need to obtain a continuous representation of any state-action pair $(s, a)$. This representation should incorporate both the combinatorial nature of graph $G$ and the structure of a solution $L$. Considering these factors, we adopt the message passing neural networks (MPNN) architecture \cite{gilmer2017neural}, which is a general graph neural network framework to obtain node representations by collecting information iteratively from local graph structures. In detail, we first initialize an embedding vector $\mu_v^0=\bm{0}\in\mathbb{R}^{d}$ for each node $v$; then at round $k$, $\{\mu_v^k\}$ is updated by leveraging information from its neighbors by:
% \begin{tiny}
\begin{equation}\label{eq:graph-encoder}
\begin{aligned}
    \mu_v^{k+1}=\text{relu}\Big(\theta_0 x_v + \theta_1 \frac{1}{|N(v)|}\sum_{u\in N(v)}w_{uv}\mu_u^k \\+ \theta_2 \frac{1}{|N(v)|}\sum_{u\in N(v)}\text{relu}(\theta_3 w_{uv})\Big),
\end{aligned}
\end{equation}
% \end{tiny}
where $\theta_0, \theta_2 \in \mathbb{R}^{d\times p}, \theta_1 \in \mathbb{R}^{d\times d}$ and $\theta_3 \in \mathbb{R}^p$ are model parameters, $N(v)$ is the set of node $v$'s neighbors and $|N(v)|$ is its cardinality. In the first term, $x_v \in \mathbb{R}^p$ is the static feature vector for vertex $v$ that incorporates additional node information from a problem instance. For instance, in Maximum $k$-Cut, $x_v$ can take the form of a one-hot label vector of $v$ to encode the current cut information; and in TSP, $x_v$ can be the initial coordinates of $v$ if given. The second term in Eq \eqref{eq:graph-encoder} aims to aggregate information from $v$'s neighbors by taking a weighted average over the neighbors' embeddings proportional to the edge-weights. This encodes neighborhood information together with their edge weight defined relatedness. And the third term is served to emphasize if $v$ is closely connected to its neighbors based on the given edge weights. 
%Compared to the GNN structure employed in S2V-DQN, there are two main differences in our design: First. we replaced the vanilla average in the second term with a weighted one, which better captures the local structure; 2. we scale the second and the third term with a constant factor $\frac{1}{|N(v)|}$, which, based on our observation, plays an essential role in the generalization to larger problem instances. 

The final node embeddings $\{\mu_v^{T}\}$ are obtained by iterating this procedure for $T$ rounds, such that they are expected to carry $T$-hop information among the nodes based on the graph topology. The state and action representations can thus be constructed based on the computed node embeddings $\{\mu_v^{T}\}$. For different COPs, we need different readout functions to compute the graph embedding from node embeddings. Take Maximum $k$-Cut and TSP as two examples to illustrate this process.

\noindent{\textbf{$\bullet$ Maximum $k$-Cut}}, suppose the current graph cut given by state $s=(G,L)$ is $(V_1, \cdots, V_k)$, where each $V_i$ corresponds to a cluster of nodes. We first define the cluster representation by averaging all the node vectors within the cluster as $H_c(i)=\frac{1}{|V_i|}\sum_{v \in V_i} \mu_v^{T}$. For the action embedding, we represent a flipping action (i.e., to flip $u$'s label from $i$ to $j$) as the concatenation $H_a^{flip}=[\mu_u^{T}; H_c(j)]$, where $\mu_u^{T}$ is the representation of vertex $u$, which is expected to carry information about vertex $u$ and cluster $i$, and $H_c(j)$ is the representation of the target cluster $j$. Similarly, we can also define the representation of the swapping action (i.e., to swap the labels of $u$ and $v$) as $H_a=[\mu_u^{T}; \mu_v^{T}; H_c(l(u)); H_c(l(v))]$, where $l(u)$ and $l(v)$ correspond to $u$ and $v$'s current labels. Finally, we use attention to construct the state representation over cluster embeddings. The attention weight is computed by taking cluster embeddings as the reference and the action embedding as the query: $w(i) = \text{softmax}_i(H_c^\top(i)W_a H_a)$,
where $H_c(i) \in \mathbb{R}^{d}, H_a \in \mathbb{R}^{4d}$, and $W_a \in \mathbb{R}^{d\times 4d}$ is a trainable parameter matrix. Then the state representation is formed by $H_s=\sum_{i=1}^{k} w(i)H_c(i)$.

\noindent{\textbf{$\bullet$ TSP}}, its solution exhibits a sequential structure instead of a clustered one. Therefore, we adopt an RNN encoder to get the state embedding: $H_s = RNN(\{\mu^T_i\}_{i=1}^n;\Theta^{RNN})$, where $\{\mu^T_i\}_{i=1}^n$ is the sequential input of RNN defined by the node permutation in solution $L$, $\Theta^{RNN}$ is the weights of RNN, and the output $H_s$ is taken as the RNN hidden state at step $n$. Because of the constraint in TSP, i.e., no repeated nodes on a tour, flipping action does not apply. To specify the swapping action, we define the sequential-swap $(i, j), i<j$, for TSP as to swap the sub-sequence $(L_i, L_{i+1}, \cdots, L_j)$ in $L$ to $(L_j, L_{j-1}, \cdots, L_i)$. Because a sequential-swap action $(i, j)$ only changes edge-weights associated with $v_{i-1},v_i, v_j,v_{j+1}$ in the TSP tour (i.e., change edges from $v_{i-1,i}, v_{j,j+1}$ to $v_{i-1,j}, v_{i,j+1}$), we represent it by $H_a=[\mu_i^{T};  \mu_j^{T}; \mu_{i-1}^{T}; \mu_{j+1}^{T}]$, where $1\leq i<j\leq n, \mu^T_0=\mu^T_n, \mu^T_{n+1}=\mu^T_1$. 

Based on the state and action representations, we establish the parameterized Q-function as $Q(s, a)=W_0 \cdot \text{relu}([W_1H_s; W_2H_a])$, where $W_0 \in \mathbb{R}^{1 \times 2d}, W_1\in \mathbb{R}^{d\times d_s}, W_2\in \mathbb{R}^{d\times d_a}$ are trainable parameters, $d_s$ and $d_a$ are the dimensions of state and action embeddings respectively. We use swap action design in Maximum $k$-Cut as an example in Algorithm \ref{q-learn} to illustrate the procedure of applying our proposed RL solution framework for COPs.

\subsection{End-to-End Training}\label{end2end}
We apply $N$-step off-policy TD method \cite{sutton2018reinforcement}, i.e., $N$-step Q-learning to train $Q(s, a)$, which has been demonstrated to be effective when dealing with delayed rewards. By evaluating the value function $N$-step ahead, we encourage the agent to be less myopic by avoiding eagerly punishing an action which induces a negative immediate reward. At each training step, we first sample a random batch of state-action-reward tuples $\mathcal{B}\!=\!\big\{(s^0_1, \{a^j_1\}_{j=1}^N, \{r_1^j\}_{j=1}^N, s^N_1), \cdots, (s^0_b, \{a_b^j\}_{j=1}^N, \{r_b^j\}_{j=1}^N, s^N_b)\big\}$ from the replay buffer $\mathcal{M}$, where the index $j=1,\cdots,N$ denotes the observations at the $j$-th step from the corresponding state $s^0$. The q-loss is given by $\sum_{i=1}^b\big(y_i\!-\!Q(s_i, a_i; \Theta)\big)^2$, where the target $y_i$ is computed as the accumulated reward in $N$ steps starting from $s^0_i$ and plus the estimated long-term rewards starting from $s_i^N$:
\begin{equation}\label{q-tar}
    y_i = \sum_{j=1}^N \gamma^{j-1} r_i^j + \gamma^N \argmax_a Q(s_i^N,a;\hat{\Theta}),
\end{equation}
where $\gamma\!\in \!(0, 1)$ is the discounting factor and $\hat{\Theta}$ is the currently estimated parameter in the target Q-net.

%\begin{figure}
%\centering
%\includegraphics[width=1.0\textwidth]{resource/dqn_illus.png}
%\caption{\label{fig:dqn_struct}The DQN architecture for Maximum $k$-Cut}
%\end{figure}

\begin{algorithm}[t]\label{q-learn}
\SetKwInOut{KIN}{input}
\SetKwInOut{KOUT}{output}
\caption{Q-learning for swap search}
\KIN{Training epochs $E$, episode maximum length $M$, exploration constant $\varepsilon$}
\KOUT{Model parameter $\Theta$}
Initialize experience replay buffer $\mathcal{M}$\\
\For{$epoch \leftarrow 1$ to $E$} {
    Sample a graph $G(V, w)$ from $\mathcal{D}$.\\
    Initialize a random solution $L_0$.\\
    \For{$t \leftarrow 0$ to $T$} {
        with probability $\varepsilon$, select a random node pair $a_t = (v_i, v_j)$; \\othereise, $a_t=\text{argmax}_{(i,j)}Q(s_t, (v_i, v_j);\Theta)$.\\
        % $a_t =$ 
        % \left\{  
        %   \begin{array}{lr}
        %  $\text{select a random node pair } $ ($v_i$, $v_j$), with probability $\varepsilon$;\\
        %  \text{argmax}$_{(i,j)}Q(s_t, (v_i, v_j);\Theta)$, otherwise.
        %     \end{array}  
        %  \right . \\
        Swap the $i$-th and $j$-th elements in $L_t$ to give $L_{t+1}$, assign $s_{t+1}=(G, L_{t+1})$, \\
        Execute the evaluation function $O(G, L_{t+1})$ to observe reward $r_t$.\\
        \If {t $\geq$ N} {
        Add tuple $(s_{t-N}, a_{t-N}, r_{t-N,t}, s_{t})$ to $\mathcal{M}$, \\
        Sample a batch $\mathcal{B}$ from $\mathcal{M}$,\\
        Update $\Theta$ for $\mathcal{B}$ via gradient descent.}
        }
    }
\end{algorithm}

The main challenge for Algorithm \ref{q-learn} lies in the evaluation of optimal action in planning: computing the maximum of $Q(s, a)$ over all actions in Eq \eqref{q-tar} could be extremely expensive, especially when we adopt the swapping action space $\mathcal{A}^{swap}$ design, which is of size $O(n^2)$ and $n$ is the number of nodes. In this case, the time and space complexity for a single forward operation is $O(n^2d^2)$ and $O(n^2d)$ respectively, where $d$ is the hidden dimension of state representation. Inspired by \cite{van2020q,dulac2015deep}, we introduce an auxiliary action-proposal network to perform action elimination. The idea is that after the state embedding $H_s$ is obtained for the current state $s$, we directly propose a pseudo action $\Tilde{a}(s)$ in $\mathbb{R}^d$ from the auxiliary network: $\Tilde{a}(s) \!= \!AP(H_s;\Theta_{ap})$.

Although $\Tilde{a}(s)$ might not directly map to a real action, $\Tilde{a}(s)$ is expected to lie around the optimal action in state $s$. Therefore, we can generate a distribution $\pi^{prop}(a)$ over the whole action space 
%$\mathcal{A}^{swap}=\{a=(v_i, v_j)| i<j, l_i\neq l_j \}$ 
by leveraging the similarity between $\Tilde{a}(s)$ and each node's embedding $\mu^T_v$. For example, for swapping actions, we set $\pi^{prop}(v_i, v_j)\! \propto \!\exp\big(s(v_i)\! +\! s(v_j)\! + \!\theta_0 s(v_i) s(v_j)\big)$, where $s(v) \!=\! \Tilde{a}(s)^\top \mu^T_v$ and $\theta_0\! \in\! \mathbb{R}$ is a trainable parameter. 
To perform action elimination, we first choose an action reserve ratio $\epsilon \!\in\! (0, 1]$, then draw a subset $\mathcal{A}^{swap}_{prop}$ of size $\epsilon|\mathcal{A}^{swap}| \!\propto \!O(n)$ from $\mathcal{A}^{swap}$ according to $\pi^{prop}(a)$, and restrict the search space of actions in Eq \eqref{q-tar} to $\mathcal{A}^{swap}_{prop}$. By deploying the auxiliary action proposal network, we reduce the time and space complexity for a single forward operation to $O(n^2\!+\!nd^2)$ and $O(n^2\!+\!nd)$. In practice, we observe that the hidden dimension $d$ should always increase proportionally to $n$ in order to guarantee good empirical performance. And this action elimination technique is essential to make the RL framework applicable to large-scale COPs.

To train the action proposal network, we introduce a regularized loss function:
\begin{equation} \label{prop_loss}
    \mathcal{L}(\Theta_{ap}; s)=-\log \pi^{prop}(a^*(s)|\Theta_{ap}) -\lambda H(\pi^{prop}(a|\Theta_{ap})),
\end{equation}
where $a^*(s) = \argmax_{a \in \mathcal{A}^{swap}_{prop}} Q(s,a;\hat{\Theta})$ is the action selected by the Q-net among the proposed action set $\mathcal{A}^{swap}_{prop}$. The first term in Eq \eqref{prop_loss} is to minimize the negative log-likelihood for the selected action, which makes the action with the highest Q-value more likely to be proposed. The second term is the negative entropy of the proposal distribution, and minimizing it would encourage uncertainty in $\pi^{prop}$ throughout training and prevents it from collapsing to a deterministic distribution.



%\begin{table}
%\centering
%\begin{tabular}{c|c|c}
%cost & time & space \\\hline
%Without A.P. Net.& $O(n^2d^2)$ & $O(n^2d)$\\
%With A.P. Net.& $O(n^2 + nd^2)$ & $O(n^2 + nd)$
%\end{tabular}
%\caption{\label{tab:time reduce}Time and space complexity reduction after applying action proposal network.}
%\end{table}

% \subsection{Active Searching}




==> NeurIPS2020/related.tex <==
\section{Related Works}

The recent success of applying machine learning to solve COPs can be traced back to \citet{vinyals2015pointer}, where pointer networks are used to solve TSP via supervised learning. Then \citet{bello2016neural} further developed an RL solution for TSP based on pointer networks using policy gradient. After that, a number of follow-up works emerged to focus on various COPs with different challenges. For example, \citet{kool2018attention} applied the Transformer architecture as the state encoder and reported state-of-the-art results on vehicle routing problems. \citet{ma2019combinatorial} resorted to a hierarchical RL structure to address TSP with time-window constraints. And \citet{abe2019solving} trained a GCN with Monte-Carlo tree search to enhance its generalizability on five NP-hard COPs. Besides these attempts, S2V-DQN \cite{khalil2017learning}, to the best of our knowledge, is the first general RL-based solution for COPs. It combines a graph neural network (GNN) and deep Q-network and is demonstrated to be effective across three classes of COPs (i.e. Minimum Vertex Cover, TSP, and Maximum 2-Cut). 

All the aforementioned RL-based methods employ a greedy node selection strategy to construct solutions, i.e., classifying one unlabeled node at a time until all nodes are labeled. Instead of constructing the solution in an incremental manner, \citet{ecodqn} proposed ECO-DQN for Max Cut, an exploratory method that allows the RL agent to continuously improve any given solution via local search \cite{johnson1988easy}, by modeling the actions as vertex-flipping. This distinctive reversible action design enables the agent to access any valid solution during planning. The reported empirical improvement from this reversible action design suggests its advantage over its irreversible counterpart.  
%They named the RL agents in ECO-DQN and those in former RL formulations as reversible/irreversible ones accordingly and claimed a remarkable improvement of reversible agents compared to irreversible ones. 
However, ECO-DQN involves several ad-hoc designs in its modeling pipeline (such as reward shaping and input feature engineering), which makes it less applicable to other COPs. 

% However, the generalizability of ECO-DQN seems to be limited due to two observations. First, the vertex-flipping action design only applies to COPs with simple solution structures, e.g. Maximum 2-Cut. For problems like Maximum $k$-Cut ($k>2$) and TSP, the algorithm design pattern cannot trivially generalize.

% Apart from value-based and policy-based RL, another direction is applying GNN with a tree search: \cite{li2018combinatorial} utilized a GCN along with a guided tree-search in a supervised manner on four canonical NP-hard problems, and , \cite{abe2019solving} trained a GCN with Monte-Carlo tree search as a boosting module.




==> algorithm.tex <==
\section{Learning from Explorative Users' Revealed Preferences}\label{sec:algo}

%First, we present the system's strategy from a high level. Since the system only observes binary decisions from the user, the only way to identify the best arm is to track the history of recommendations and rejections in order to eliminate suboptimal arms. 
With stochastic rewards, we know $\mathbb{P}[\mu_i \in CI_{i,t}]$ almost always increases as the number of acceptances $n(t)$ grows. Therefore, the system can confidently  rule out a sub-optimal arm once it has collected a reasonable number of acceptances. In light of this, we devise a two-phase explore-then-exploit strategy for system learning: the system first accumulates a sufficient number of acceptances and then examines through the arm set to eliminate sub-optimal ones with a high confidence. % Next, we present the algorithm for the two phases in detail.

\begin{algorithm}[t]
   \caption{Phase-1 Sweeping}
   \label{alg:phase1_alg}
%   \begin{multicols}{2}
\begin{algorithmic}
   \STATE {\bfseries Input:} $K>0$, $\delta\in (0,1) ,N_1(\delta)>0$. 
%   \REPEAT
\STATE {\bfseries Initialization:} $F=[K]$,$ N=0, n_i=0, i\in[K].$

\REPEAT
    \STATE Recommend each item in $F$ once, and remove the rejected ones from $F$.
\UNTIL{$F$ is empty or the time step exceeds $N_1(\delta)$.}

\REPEAT
\STATE If $F$ is empty, reset $F= \{1,\cdots, K\};$
    \FOR{$i \in F$} 
    \STATE Recommend $i$ until rejected, then remove it from $F$.
\ENDFOR
\UNTIL{The time step exceeds $N_1(\delta)$.}

   \STATE {\bfseries Output:} number of acceptances for each arm $\{n_i\}_{i=1}^K$. 
\end{algorithmic}
% \end{multicols}
\end{algorithm}



\begin{algorithm}[t]
   \caption{Phase-2 Elimination}
   \label{alg:phase2_alg}
%   \begin{multicols}{2}
\begin{algorithmic}
   \STATE {\bfseries Input:} $K>0$, $\{n_i\}_{i=1}^K$ from Phase-1.
   \STATE {\bfseries Initialization:} $F=[K] $.
   \
   
   \WHILE{$|F|>1$}
   \STATE Recommend $a_t=\arg\min_{i\in[K]} n_i$ and update $n_{a_t}$.
   \STATE Remove $a_t$ from $F$ if rejected.
   \ENDWHILE
 
   \STATE {\bfseries Output:} $F$.
\end{algorithmic}
% \end{multicols}
\end{algorithm}

% \end{multicols}


The Phase-1 design is presented in Algorithm \ref{alg:phase1_alg}. Like standard bandit algorithms,  
%the system recommends each arm once to the user. Given our user behavior model, the user always accepts the first $K$ recommendations. Then, 
the system will execute an initialization procedure by sweeping through the arm set $F=[K]$ and then recommend each arm repeatedly until it collects exactly one rejection on each arm there.  This initialization stage is similar to the round-robin style pulls in  standard bandit algorithms (e.g., UCB1, $\epsilon$-Greedy). But the key difference is that our algorithm will initialize by collecting one rejection on each arm whereas standard bandit algorithm will initialize by collecting one pull (i.e., acceptance) on each arm. This is because rejections in our setup are more informative than acceptances to the system. % as the system only starts to compare arms after they have been rejected: it can never hope to differentiate those arms which have always been accepted. If the number of acceptances exceeds $N_1$ during the warm-up stage, Algorithm \ref{alg:phase1_alg} terminates. Otherwise, 
After initialization, Algorithm \ref{alg:phase1_alg} enters the main loop and do the following: keeps recommending the same arm until it gets rejected and then moves to another arm in $F$. After each arm gets rejected once, the system starts a new round by resetting $F=[K]$. This procedure continues until the total number of acceptances exceeds $N_1(\delta)$. 
This sweeping strategy reflects the principle of Phase-1: the system aims to collect a reasonable number of acceptances while minimizing the number of rejections by not recommending any risky arm. 
For the ease of analysis, we divide Phase-1 into different \emph{rounds} (indexed by $r$) by the time steps when the system resets $F$.  We will prove later that there is a tailored choice of $N_1(\delta)$ such that when the system enters Phase-2 with $N_1(\delta)$ acceptance, it can identify the best arm with probability $1-\delta$. %The detailed discussion will be presented in the next two subsections. Next, 


We now present the design for Phase-2, as shown in Algorithm \ref{alg:phase2_alg}, which follows Phase-1 Sweeping. Here, the system executes arm elimination: always recommend the arm with the minimum number of acceptances; and eliminate an arm when it is rejected by the user, until there is only one arm left. We prove that the stopping time of Algorithm \ref{alg:phase2_alg} is finite with probability 1, and it outputs the best arm with probability $1-\delta$ when it terminates. We name our proposed two-phase algorithm  \textbf{B}est \textbf{A}rm \textbf{I}dentification under \textbf{R}evealed preferences, or BAIR for short. 

Next, we analyze BAIR by upper bounding its stopping time given fixed confidence $\delta$. Our main result is formalized in the following theorem.

\begin{theorem}%[The Upper Bound for BAIR]
\label{thm:upperbound2}
When $\Gamma$ is defined as in Eq \eqref{eq:trust}, with probability at least $1-2\delta$, the system   makes at most $$  O\Big(K^{\frac{1}{\alpha}}\delta^{-\frac{1}{\alpha}}+K^{1+\frac{1}{2\alpha}}\delta^{-\frac{1}{2\alpha}}\sqrt{\log\frac{K}{\delta}}+\frac{\alpha K}{\Delta_1^2}\log\frac{ K}{\delta \Delta_1}\Big)$$ recommendations and successfully identifies the best arm by running Algorithm \ref{alg:phase1_alg} and \ref{alg:phase2_alg}. 
\end{theorem}
Note that the upper bound on the number of rounds above is deterministic while not in expectation. The proof of Theorem \ref{thm:upperbound2} requires separate analysis for Phase-1 and Phase-2, which we discuss in the following subsections. At a high level, the first two terms in the bound come from the number of acceptances and rejections in Phase-1, and the last term corresponds to the number of acceptances in Phase-2. We decompose the bound in Theorem \ref{thm:upperbound2} in Table \ref{tb:upperbounds}.
\begin{table}[ht]
\vspace{-1mm}
\centering
\caption{Upper bounds on \#recommendations in Phase 1,2}
\begin{tabular}{c|c|c|c}
 \hline
 Phase & \# Acceptance & \# Rejection &  Prob. \\  \hline
 1 & $O(K^{\frac{1}{\alpha}}\delta^{-\frac{1}{\alpha}})$ & $O(K^{\frac{1+2\alpha}{2\alpha}}\delta^{-\frac{1}{2\alpha}}\log^{\frac{1}{2}}\frac{K}{\delta})$ & $1-\delta$ \\  \hline
 2 & $O(\frac{\alpha K}{\Delta_1^2}\log\frac{K}{\delta \Delta_1})$ & $K$ & $1-\delta$ \\ \hline
\end{tabular}
\vspace{-2mm}
\label{tb:upperbounds}
\end{table}

Note that there is a clear \emph{tradeoff} between the upper bounds in Phase-1 and Phase-2 in terms of $\alpha$: a smaller $\alpha$ increases the upper bound in Phase-1 but requires less number of recommendations in Phase-2, while a larger $\alpha$ ensures a lighter Phase-1 but would result in a more cumbersome Phase-2. This is expected because, e.g., when facing a highly explorative user (large $\alpha$), the system can easily accumulate sufficient acceptances in Phase-1. However, it will need more comparisons in Phase-2 to identify the best arm for such a highly explorative user. Theoretically, there exists an optimal $\alpha$ which minimizes the total number of recommendations; however, this is not particularly interesting to investigate in this paper, as $\alpha$ is not under the system's control, but a characterization of the user.

%the system has to spend more time in Phase-1 to accumulate sufficient explorations when facing a conservative user; on the other hand, it needs more comparisons in Phase-2 to identify the best arm when the user is highly explorative. Theoretically, there exists an optimal $\alpha$ which minimizes the total number of recommendations; however, this is not particularly interesting to investigate in this paper, as $\alpha$ is not under the system's control, but a characterization of the user.

% In the following sections, we will analyze BAIR by upper bounding its stopping time given fixed confidence $\delta$ for Phase-1 and Phase-2 separately. 


==> author_response.tex <==
\newpage

\noindent 
We thank all reviewers for their constructive comments. In the following, we first respond to two questions in common and then respond to each individual reviewer's comments. 

\noindent\textbf{Global response: \textit{Is it possible to test BAIR using real datasets?}} We fully agree this is an intriguing direction, however the focus of this work is to develop a theoretical solution for a novel problem setup where the user is learning and to study how this user learning behavior urges for new designs in recommendation algorithms. As the first attempt in this direction, we believe our work is already a significant step forward from existing recommendation solutions, most of which simply assumed users have full information regarding the recommendation candidates beforehand. 
On the other hand, real-world evaluation is highly non-trivial, and is an important future direction we plan to pursue. Given the lack of access to a population of real users, we have to resort to offline logs, i.e., off-policy evaluation. But since existing public datasets merely contain interaction records generated by methods that do not consider the explorative user behavior, they are likely to miss the best arm. As a result, the choice from our algorithm may not be rewarded even if it finds the best one, simply because it is not recorded in the dataset. 
\textit{\textbf{Ethical discussions.}} Our system is helping the user to realize her best options from a large collection of candidates. Without the system's help, the user would have to do everything by herself. Moreover, we should note the choice is on the users to accept or reject the recommendation: when the user rejects, the system gets penalized. According to our experiment, BAIR enjoys the least fraction of rejections compared to other baseline algorithms, i.e., higher user satisfaction about the recommendations. 
% \hf{Is this a common concern? Only R4 has it? Putting it here may make other reviewers to re-think about this issue, which may not be a good thing for us. }

\noindent 
\textbf{R2: \textit{Why BAIR can remedy the mentioned issues?}} As discussed in Section 4.3, the failure of the baseline algorithms is due to the lack of exploration when facing an explorative user. 
%On the contrary, the success of BAIR is because of the sufficient exploration from the beginning.  
BAIR does not assume independent or stationary user responses; instead, it exploits the fact that an explorative user's responses become more reliable until the exploration is sufficient, which yields its two-phase recommendation strategy and corresponding theoretical guarantees. Or more specifically, in Phase-1, BAIR provides as comprehensive exploration as possible while maintaining user's satisfaction (by minimizing the number of rejections). And in Phase-2, when the exploration is sufficient, BAIR follows the user's preference to match her with the best choice.


\noindent 
%\textbf{R3: \textit{Why classical practice assumes users to be omniscient, static, and explicit.}} 
\textbf{R3: \textit{Assumptions in existing RS algorithms?}} We believe that any RS algorithms based on supervised learning has to (explicitly or implicitly) assume users have the full information beforehand, as their training labels are derived from users' feedback. They just have different noise and observation assumptions. For example, almost all existing RS algorithms based on matrix factorization, neural networks or their variants fall into this category (e.g., using clicks, purchase, ratings for model training). 
We should also clarify that the terms \emph{explicit} and \emph{implicit} used in our paper do not refer to the contrast between numerical ratings and click/non-click feedback. We use \emph{explicit} feedback to refer to the assumption that user's response truthfully reflects the utility of the recommendation (e.g., true quality of the item), which we believe is only possible after the user consumes the recommendation. 
%In contrast, \emph{implicit} feedback means the response is given by comparison and does not necessarily imply the user’s true utility over a specific item. 
We will make this point clearer in the final version. \textit{\textbf{Any recent baselines?}} For the problem of best arm identification with fixed confidence, to the best of our knowledge, the Track-and-stop is the optimal algorithm in terms of efficiency as it has a matching lower bound guarantee. For EXP3, there are some variants such as EXP-IX which targets on improving the high probability regret guarantee. But as we explained in the experiment section, the failure of EXP3 is due to the mismatched user behavior assumption, and thus cannot be fixed by an algorithm with slightly improved regret guarantee. 
Hence the negative result for EXP3 well represents the performance of a broad class of adversarial bandit algorithms in our problem setting. \textit{\textbf{Reward assumptions.}} We remark what important to our results are only the independence and sub-Gaussian assumptions, which are quite standard in online learning and bandit literature.  %Independence models the situation where rewards reflect the intrinsic property of the recommended item. The sub-Gaussian distribution is popularly used in bandit algorithms, as it is a very general class of probability distributions including the entire exponential family and beyond. 
Notably, the unit variance assumption (1-sub-Gaussian) is \emph{without loss of generality} and is merely assumed for notational convenience. It can be replaced with any bounded variance $\sigma$, with the corresponding regret rescaled linearly by   $\sigma$.  This is because for any bounded variance we can rescale the reward such that the variance is 1. 

\noindent 
\textbf{R4: \textit{Why best arm?}} First, we remark that the goal of best arm identification (BAI) is aligned with regret minimisation: any fixed-confidence BAI algorithm can be easily converted to an explore-then-commit regret minimisation algorithm with an optimal order-wise regret guarantee (see, e.g., ``On Explore-Then-Commit Strategies'', Garivier et al., 2016). Second, BAI is well-motivated for recommender systems (e.g., ``Best-Arm Identification in Correlated Multi-Armed Bandits'' by Gupta et al., 2021): such a system helps the users consume the high-utility items as often as possible. 
%From a long-term point of view, this objective is optimized when the system finds the best arm, i.e., a user’s favorite category of items. 
\textit{\textbf{Why pulling the same arm repeatedly?}} We remark that ``pulling an arm''  should be   interpreted as ``recommending a certain \emph{category} of items'' in practice. Therefore, finding the best arm means learning the most attractive item type or category for a user. We elaborated this point in Appendix A and will further clarify this in the final version. 
\textit{\textbf{Tightness of our result.}} We focused primarily on the tightness in $\delta$ because this was most studied in previous BAI problems and it is intrinsically related to the PAC-learnability of the problem. However, it is indeed interesting to examine tightness w.r.t   $K$ as well. Any succcessful MAB algorithm must use $\Omega(K)$ rounds as it has to pull each arm at least once whereas BAIR's dependency on $K$  is $O(K^{1.5})$ as mentioned at the end of Section 4.3. Closing this gap is an open problem.   
%Therefore, the gap between our lower and upper bounds is $O(\sqrt{K})$. Our empirical result shows that the stopping time of BAIR does depend on $K$ linearly; and thus how to tighten the upper bound is still an open problem. We will make this discussion clearer in the final version. 
\textit{\textbf{Is the best arm ever rejected in Phase-1?}} The best arm can be rejected in Phase-1 due to the inaccuracy of the user's confidence interval. Note that only when $t$ is sufficiently large, the UCB-type confidence interval contains the true parameter with arbitrarily high probability. This is exactly why we need sufficient exploration in Phase-1 to avoid such bad cases. %We will elaborate more on this aspect in the main text. 
\textit{\textbf{Binary feedback.}} 
% \hf{I do not think we need to answer this question --- the reviewer already said that he saw the novelty of our model, and just thought that we could write better. He is already giving an accept to our paper, so we could just say at the very begining "we appreciate the reviewer's suggestion on the writing and  will make the change accordingly.  I think there is no point to argue with him that "look, your point was not accurate" --- what is the goal for us to argue with him? I  think it is unlikely to get him to increase to a "strong accept" anyway.... } 
We did not mean to emphasize the novelty of binary feedback. In fact, we are proposing a new way to interpret the binary feedback: 1) it is modeled as users' comparison among the recommendation candidates, 2) it is not even clear to the system what the reference is in the observed comparisons. We will clarify it more in the final version.

% We believe this is a more realistic yet challenging modeling of users' feedback  that previous works did not consider.  

% \textbf{I find the user model (the paragraph of "The decision rule") as a crucial part of the formulation, but this part gets lost in the text (this also relates to my initial confusion about "why is it not just Bernoulli samples of the reward" when reading the introduction). I suggest re-writing the formulation as the "system-side model" (similar to the current steps 1-3 in Section 2), and the "user-side model"; the simulation results (Tables 1 and 2) are more readable if presented as figures; in simulation, the paper should be more clear how the binary feedback is used in the existing algorithms (Track-and-stop and EXP3). I assume the binary feedback is naively used as a binary reward.}  
% Thanks for the detailed suggestions and we will carefully revise the final version accordingly.


==> cover.tex <==
\newpage

\noindent
Dear JMLR reviewers:

We are pleased to submit our manuscript titled “PAC-learning for Strategic Classification” to JMLR. We believe that our result will be of general interest to the readership of the journal as well as the adversarial machine learning community. 

This submission is an extended version of our conference paper \cite{sundaram2021pac}, which has been accepted by ICML2021 as a long presentation. Our work \cite{sundaram2021pac} proposes a new strategic classification setting where agents have heterogeneous strategic preferences. We propose a new concept, strategic VC-dimension (SVC), to sketch the PAC-learnability of this type of strategic classification problem. As a case study, we also characterize the statistical learnability and computational tractability for the class of linear classifiers. Our current submitted manuscript includes all the results from \cite{sundaram2021pac}, and a new section discussing the power of randomization under our strategic setting. Our new result discloses an observation that randomization only helps when the manipulations come with costs. This observation is particularly interesting because it implies that randomization (over linear classifiers) does not help in standard adversarial classification with zero-manipulation-cost. We hope this additional discussion enriches our study of strategic classification under heterogeneous preferences and might open up a re-thinking over randomized classifiers in strategic environments. 

We confirm that all co-authors (Ravi Sundaram, Anil Vullikanti, Haifeng Xu, Fan Yao) are aware of the current submission and consent to its review by JMLR.

\fan{Required content in the cover letter by the JMLR submission instruction:
\begin{enumerate}
    \item Disclosure of any previous publications by the author(s) that significantly overlap with the submission. E.g., if the submission is an extended version of an earlier conference paper, please described the differences between the two papers.
    \item Confirmation that all co-authors are aware of the current submission and consent to its review by JMLR.
    \item Declaration of possible conflicts of interest; in particular, name all action editors that have recently collaborated with authors of the submission.
    \item Suggestions of 3 to 5 action editors that seem best suited to handle the submitted manuscript. These suggestions will be considered (though not necessarily honored). We have found that some action editors are popular with many authors, and may be busy handling other papers at a given point in time, so listing at least three action editors helps us expedite the process.
    \item Suggestions of 3 to 5 reviewers. These suggestions will be considered (though, again, not necessarily taken) by the action editor. As a reminder, do not suggest reviewers for whom there is a conflict of interest. 
\end{enumerate}
}





==> discussion.tex <==
\section{Discussions and Future Work}\label{sec:discussion}

To bring user modeling to a more realistic setting in modern recommender systems, we proposed a new learning problem of best arm identification from explorative users' revealed preferences. We relax the strong assumptions that users are omniscient by modeling users' learning behavior, and study the learning problem on the system side to infer user's true preferences given only the revealed user feedback. We proved efficient system learning is still possible under this challenging setting by developing a best arm identification algorithm with complete analysis, and also disclosed the intrinsic hardness introduced by the new problem setup. Our result illustrates the inevitable cost a recommender system has to pay when it cannot directly learn from a user's realized utilities. As concluding remarks, we point out some interesting open problems in this direction:
%\begin{itemize}[leftmargin=*]
    
\noindent\textbf{The optimal choice of $N_1$.} 
Although our lower bound result in Theorem \ref{thm:lowerbound4delta} is tight in $\delta$, it does not match the upper bound in Theorem \ref{thm:upperbound2} in terms of $K$. The mismatch comes from the choice of $N_1=(2K/\delta)^{1/\alpha}/\rho_0$, which might be overly pessimistic as Theorem \ref{thm:lowerbound4delta} only indicates a necessary condition of $N_1>\delta^{-1/\alpha} / \rho_0$. To bridge this gap, a tighter upper bound is needed to improve the choice of $N_1$. We believe this is promising because the experiment results in Table \ref{tb:exper-baselines} demonstrate that the choice of $N_1=(2K/\delta)^{1/\alpha}/\rho_0$ almost guarantees a success probability $1.0$ even when $\delta$ takes a large value, e.g., $0.1$. This implies the stopping time of BAIR could be improved by setting a smaller $N_1$. In practice, we can fine-tune $N_1$ to pin down the optimal choice. For example, one can simply apply binary search within $(0, (2K/\delta)^{1/\alpha}/\rho_0)$ with $N_1=O(\delta^{-1/\alpha})$ as a starting point. 

% \noindent\textbf{The design of trust function.} 
% Our current trust function captures a wide range of possible user behavior but does not explicitly penalize the system when it receives too many rejections. In real applications, making bad recommendations will probably lead to more serious reactions from the user, than just becoming more conservative on the system's recommendations (e.g., leave the system or become stochastic in responses). To design a more realistic trust model by integrating an explicit penalty module could be another interesting future direction. 

% \noindent\textbf{Utility-driven user modeling.} 
% Our work provides a useful insight to the designer of a recommender system. Instead of observing user responses as the actual preferences, it is more reasonable to interpret them as the revealed preferences under a specific behavior model. The behavior model we proposed in Section \ref{sec:usermodel} is not necessarily the only option. We can go beyond the current UCB-based design and consider a more general setting where the user is driven by an underlying utility function. Since the system is to optimize some long-term objective, this type of utility-driven user modeling allows us to study the interactions between the system and the user under a game theoretical framework, which happens to be a repeated Stackelberg game in this case. Moreover, this general framework makes it possible to consider richer behaviors, e.g., the system and the user are not cooperative or even strategically against each other. %We plan to investigate this direction in future work. 

\noindent\textbf{Beyond a single user.}
We note that our problem formulation and solution for the system and a single user also shed light on learning from a \emph{population} of users. For example, users sometimes learn or calibrate their utility from third-party services that evaluate the quality of items by aggregating users' feedback across different platforms.
%, e.g., Trakt for media discovery and engagement. %and Capital One Shopping for online shopping. 
As a result, users equipped with these services are inclined to exhibit an exploratory pattern and make decisions based on the comparison of confidence intervals.
% rendering the traditional omniscient yet myopic user model insufficient for the system designer. 
We believe that our problem setting also provides a prototype to study the optimal strategy for the system under this new emerging situation.
    % From Figure \ref{fig:comparison} we observe that the BAIR's probability of success is exceptionally high even when we set a mild threshold $\delta$. This might suggest that the empirical performance of BAIR can still be improved by seeking a trade-off between the stopping time and the probability of success, which can be expected by tuning $N_1$ for Phase-1: a small $N_1$ saves the system a lot of budget in Phase-1 but increases the risk of misidentifying the best arm in Phase-2; a large $N_1$ guarantees the probability of success but might waste the system too much budget in Phase-1, which is likely the main bottleneck of BAIR as $\delta \xrightarrow{} 0$. Since we showed in Lemma \ref{lm:phase2bound1} that $N_1=O(\frac{K}{\delta})$ theoretically guarantees a success probability $1-\delta$, and we know from Theorem \ref{thm:lowerbound4delta} that $N_1$ is tight in terms of $O(\frac{1}{\delta})$. Hence the question is whether there is an empirically better choice for $N_1$? In Table \ref{tb:exper-N1}, we run BAIR under the same environment setting as in Table \ref{tb:exper-baselines}, but with three different choices of $N_1=\{\frac{2K}{\delta},\frac{2}{\delta},0\}$. When choosing $N_1=0$, the system simply skips Phase-1 and runs Phase-2 elimination. And as we can find in Table \ref{tb:exper-N1}, the probability of success fails to meet the threshold $1-\delta$. However, if we choose $N_1=\frac{2}{\delta}$ instead of $\frac{2K}{\delta}$, BAIR still terminates with a high successful probability above $1-\delta$ and with a smaller stopping time. 
    % This suggests that the theoretical value $N_1=\frac{2K}{\delta}$ might be too conservative and we can expect more competitive performance of BAIR by tuning $N_1$ as a hyper-parameter. For example, we can apply grid search for $N_1$ in practice and $N_1=\frac{2}{\delta}$ could be a good starting point.
    % \item \textbf{How Phase-1 contributes to Phase-2 in BAIR.} 
    % Although the choice of $N_1=\frac{2K}{\delta}$ seems like a squander in Phase-1, it does not affect the overall performance that much simply because a longer Phase-1 leads to a shorter Phase-2. As indicated by Table \ref{tb:exper-N1}, if we compare the stopping time of Phase-2 for $N_1=\frac{2K}{\delta}$, we will find that the system spends nearly negligible time in Phase-2 compared to Phase-1 for $\delta=0.01$. The reason is that given a large $N_1$, the system has already efficiently explored all the arms during Phase-1. As a result, when it enters Phase-2, most arms have been pulled sufficiently many times and the final eliminations can thus be executed quickly. 
%\end{itemize}


% To empirically study this option, we report the stopping time of Phase-2 as well as the probability of success under different choices of $N_1$ in Table \ref{tb:exper-N1}.


% \onecolumn



% does not utilize the feedback from the early phase to make decisions but instead making safe recommendations maintain a trust 



% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{}
% \label{icml-historical}
% \end{center}
% \vskip -0.2in
% \end{figure}





% \begin{table*}[ht]
% \begin{small}
% \begin{sc}
% \caption{Comparison between BAIR and three baselines}
% \label{tb:exper-baselines}
% \begin{tabular}{ll|cc|cccc|cccc}
% \toprule
%  &   & \multicolumn{2}{c}{Stopping Time} & \multicolumn{4}{c}{Rejection Rate (\%)} & \multicolumn{4}{c}{Prob. of Success} \\
% $\delta$ & $K$ & BAIR/UNI/EXP3 & T\&S & BAIR & UNI& EXP3 & T\&S & BAIR & UNI & EXP3 & T\&S \\
% \midrule

% \multirow{5}{*}{$0.1$} & 2  & 3116 & 4516 & 0.1 & 5.4 & 0.7 & 0.1 & 0.999 & 0.737 & 0.656 & 0.998\\
%                         &  5 & 4477 & 9160 & 0.2 & 36.7 & 3.5 & 0.4 & 0.999 & 0.543 & 0.497 & 0.990\\
%                         &  20 & 9625 & 23600 & 0.4 & 49.8 & 7.6 & 9.7 & 1.000 & 0.225 & 0.463 & 0.962\\
%                         &  100 & 36613 & 57596 & 0.6 & 44.6 & 9.9 & 11.4 & 1.000 & 0.048 & 0.355 & 0.925\\
% \hline
% \multirow{5}{*}{$0.05$} & 2  & 3188 & 4555 & 0.1 &  &  & 0.1 & 0.999 &  &  & 1.000\\
%                         &  5 & 4835 & 11766 & 0.2 &  &  & 0.3 & 1.000 &  &  & 0.988\\
%                         &  20 & 9787  & 24283 & 0.4 &  &  & 9.4 & 1.000 &  &  & 0.955\\
%                         &  100 & 39415 & 60029 & 0.5 &  &  & 10.2 & 1.000 &  &  & 0.956\\
% \hline
% \multirow{5}{*}{$0.02$} & 2  & 3202 & 4602 & 0.1 &  &  & 0.2 & 1.000 &  &  & 0.995\\
%                         &  5 & 4885 & 12037 & 0.2 &  &  & 0.3 & 1.000 &  &  & 0.992\\
%                         &  20 & 9881 & 26799 & 0.5 &  &  & 8.8 & 1.000 &  &  & 0.970\\
%                         &  100 & 40626 & 66454 & 0.7 &  &  & 9.6 & 1.000 &  &  & 0.960\\
% \hline
% \multirow{5}{*}{$0.01$} & 2  & 3384 & 4623 & 0.1 &  &  & 0.2 & 1.000 &  &  & 1.000\\
%                         &  5 & 4921 & 13601 & 0.2 &  &  & 0.3 & 1.000 &  &  & 0.991\\
%                         &  20 & 10050 & 26952 & 0.5 &  &  & 8.9 & 1.000 &  &  & 0.985\\
%                         &  100 & 41885 & 69039 & 0.7 &  &  & 9.8 & 1.000 &  &  & 0.970\\
% \hline
% \multirow{5}{*}{$0.005$} & 2  & 3426 & 4683 & 0.1 & 6.7 & 0.9 & 0.2 & 1.000 & 0.791 & 0.618 & 0.997\\
%                         &  5 & 5022 & 16024 & 0.3 & 40.2 & 3.8 & 0.3 & 1.000 & 0.576 & 0.662 & 0.996\\
%                         &  20 & 10544 & 30502 & 0.6 & 50.9 & 8.0 & 8.7 & 1.000 & 0.244 & 0.508 & 0.988\\
%                         &  100 & 43868 & 82005 & 0.7 & 49.1 & 9.8 & 9.4 & 1.000 & 0.059 & 0.410 & 0.981\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \vskip -0.1in
% \end{table*}

% \begin{table*}[ht]
% \centering
% \caption{The stopping time and probability of success of BAIR under different choices of $N_1$. }
% \label{tb:exper-N1}
% \begin{small}
% \begin{sc}
% \begin{tabular}{llcccccc}
% \toprule
%  &   & \multicolumn{3}{c}{Stopping Time in Phase-2}  & \multicolumn{3}{c}{Prob. of Success} \\
% $\delta$ & $K$ & $N_1=\frac{2K}{ \delta}$ & $,\frac{2}{ \delta}$  & $,0$ & $N_1=\frac{2K}{ \delta}$ & $,\frac{2}{ \delta}$  &  $,0$ \\
% \midrule
% \multirow{5}{*}{$0.1$} & 2    & 385  & 348   & /    & 0.999 & 0.999 & /\\
% & 5                           & 657  & 621   & /    & 1.000 & 0.999 & /\\
% & 20                          & 1733 & 1867  & /    & 1.000 & 1.000 & /\\
% & 100                         & 9295 & 9260  & /    & 1.000 & 1.000 & /\\
% \multirow{5}{*}{$0.01$} & 2   & 237  & 324   & 31   & 1.000 & 1.000 &  0.706\\
% & 5                           & 140 & 657   & 207  & 1.000 & 1.000 &  0.491 \\
% & 20                          & 217 & 1927  & 734  & 1.000 & 1.000 &  0.333\\
% & 100                         & 544 & 9061 & 1753 & 1.000 & 1.000 &  0.278\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{table*}


==> experiments.tex <==
\section{Experiments}
In this section, we empirically study BAIR to support our theoretical analysis. We use simulations on synthetic datasets in comparison with several baseline algorithms. Since we propose a new perspective to model user-system interactions in RS, there is no baseline for direct comparison. However, this also gives us an opportunity to demonstrate how problematic it may be when using a wrong user model for the observed system-user interactions. 

\begin{table*}[t]
\centering
\begin{small}
\caption{Comparison between BAIR and three baselines on proposed metrics. $(\alpha=1)$}
\label{tb:exper-baselines}
\begin{tabular}{ll|cc|cccc|cccc}
\toprule
 &   & \multicolumn{2}{c}{Stopping Time} & \multicolumn{4}{c}{Rejection Rate (\%)} & \multicolumn{4}{c}{Prob. of Success} \\
$\delta$ & $K$ & BAIR & T\&S & BAIR & UNI& EXP3 & T\&S & BAIR & UNI & EXP3 & T\&S \\
\midrule

\multirow{4}{*}{$0.1$} & 2    & 405  & 539 & 0.8 & 8.5  &  2.5 & 1.0 & 0.999  & 0.786  & 0.621  & 0.999 \\
& 5                           & 737  & 1069 & 1.4 & 27.6 & 8.8  & 1.7 & 1.000  & 0.568  & 0.549  & 0.971 \\
& 20                          & 2113 & 3107 & 1.9 & 33.7 & 11.6 & 4.6 & 1.000 & 0.229  & 0.408  & 0.966 \\
& 100                         & 10449 & 16523& 2.0 & 34.4 & 13.4  & 11.9& 1.000 & 0.092 & 0.400  & 0.965\\
\hline
\multirow{4}{*}{$0.05$} & 2  & 413 & 557 & 0.7 & 9.4 & 2.8 & 1.1 & 1.000 & 0.799  & 0.654  & 1.000 \\
                        &  5 & 787 & 1123 & 1.2 & 29.2 & 7.6 & 1.9 & 1.000 & 0.599 & 0.581 & 0.978 \\
                        &  20 & 2421 & 3161 & 1.5 & 40.4 & 12.3 & 4.4 & 1.000 & 0.429& 0.577 & 0.965 \\
                        &  100 & 10826 & 16577 & 2.2 & 43.2 & 14.1 & 11.1 & 1.000 & 0.150& 0.534  & 0.945 \\
\hline
\multirow{4}{*}{$0.02$} & 2  & 422 & 544 & 0.7 & 12.2 & 3.9 & 1.2 & 1.000 & 0.806 & 0.638  & 0.999 \\
                        &  5 & 879 & 1148 & 1.2 & 31.8 & 7.7 & 2.1 & 1.000 & 0.670 & 0.607  & 0.962 \\
                        &  20 & 3593 & 3210 & 1.6 & 50.2 & 11.9 & 4.4 & 1.000 & 0.436& 0.680& 0.957 \\
                        &  100 & 11528 & 16955 & 2.5 & 46.7 & 14.2 & 12.3 & 1.000 & 0.153 & 0.634 & 0.963\\
\hline
\multirow{4}{*}{$0.01$} & 2   & 437  & 554 & 0.8 & 17.6 & 2.7 & 1.3 & 1.000 & 0.821  & 0.632  & 0.998 \\
& 5                           & 940 & 1153 & 1.3 & 34.9 & 7.7  & 2.0 & 1.000 & 0.701  & 0.604  & 0.959  \\
& 20                          & 4017 & 3223& 1.4 & 51.6 & 13.6 & 3.0& 1.000 & 0.476  & 0.737  & 0.947 \\
& 100                         & 20344& 27548 & 1.5 & 52.8 & 15.9 & 12.4 & 1.000 & 0.130  & 0.725  & 0.930 \\
\hline
\multirow{4}{*}{$0.005$} & 2   & 512 & 570 & 0.8 & 27.6 & 4.0 & 1.4 & 1.000 & 0.992  & 0.901  & 1.000 \\
& 5                            & 1692 & 1580 & 0.8 & 50.0 & 8.3 & 1.6 & 1.000 & 0.942   & 0.844  & 0.993  \\
& 20                           & 7827 & 5983& 0.7 & 71.4 & 12.4 & 5.4 & 1.000 & 0.938  & 0.921  & 0.979 \\
& 100                         & 40246 & 37931 & 0.7 & 73.1 & 15.0 & 16.0 & 1.000 & 0.794  & 0.930  & 0.970 \\
\bottomrule
\end{tabular}
\end{small}
%\vskip -0.1in
\end{table*}

\subsection{Experiment Setup and Baselines}
 
 %To come up with reasonable baselines and fair comparisons, we note that although the system faces the challenge of limited information from the user, it can always choose to treat the user as a blackbox and thus perceive the environment as an adversarial or stochastic bandit. 
 
As we discussed in the introduction, prior works treat users as an unknown but omniscient classifier, and therefore stochastic bandits are the typical choices to learn from user feedback. Moreover, since the users' responses in our problem setup are not necessarily stochastic, adversarial bandits could be another choice. Therefore, we employ the corresponding state-of-the-art algorithms, Track-and-stop \cite{garivier2016optimal} (for BAI) and EXP3 \cite{auer2002nonstochastic} (for adversarial bandits), to compare with BAIR. Besides, we also propose a heuristic baseline, uniform exploration, to directly compete with BAIR. The details of these baselines are as follows.

    \noindent \textbf{Uniform exploration (UNI)}: The system recommends candidate arms uniformly until the number of recommendations reaches the given threshold $T$. When the algorithm terminates, it outputs the arm with the maximum number of acceptances; ties are broken arbitrarily. \textbf{Track-and-stop (T\&S)}: 
    %Since the user only provides her accept/reject decisions on the recommendations, a stochastic multi-armed bandit would model the feedback on each arm as i.i.d. Bernoulli random variables. 
    This is the state-of-the-art solution for BAI with fixed confidence \cite{garivier2016optimal}. The expected stopping time of T\&S  provably matches its information-theoretic lower bound $O(\log \frac{1}{\delta})$ in the stochastic bandit setting. The effectiveness of T\&S relies on the independent and stationary reward assumptions on each arm, which fail to hold in our setup as user responses are not a simple function of their received rewards. We will investigate how the theoretical optimality of the T\&S breaks down under our problem setting. \textbf{EXP3}: 
    %When the learning environment does not guarantee the requirement for a stochastic bandit, adversarial bandit becomes a natural choice, which relaxes the assumption on the reward distribution. But, 
    To the best of our knowledge, there is no BAI algorithm under an adversarial setting. As a result, we adopt EXP3 \cite{auer2002nonstochastic} for comparison. Given the number of arms $K$ and a time horizon $T>K\log K$, EXP3 is provably a no-regret learning algorithm if taking $\gamma \sim O(\sqrt{\frac{\log K}{KT}})$ and $\epsilon \sim O(\sqrt{\frac{K\log K}{T}})$. We run EXP3 with this configuration and output the arm with the maximum number of acceptances in the end.

\begin{table*}[t]
\centering
\begin{small}
\caption{Performance of baselines with shared Phase-1. $(\alpha=1,  N_1=\frac{2K}{\delta})$}
\label{tb:exper-extra}
\begin{tabular}{ll|cc|cccc|cccc}
\toprule
 &   & \multicolumn{2}{c}{Stopping Time in Phase-2} & \multicolumn{4}{c}{Rejection Rate (\%)} & \multicolumn{4}{c}{Prob. of Success} \\
$\delta$ & $K$ & BAIR & T\&S & BAIR & UNI& EXP3 & T\&S & BAIR & UNI & EXP3 & T\&S \\
\midrule
\multirow{4}{*}{$0.02$} & 2 & 372 & 124 & 0.7 & 0.2 & 0.9 & 1.1 & 1.000 & 0.623 & 0.638  & 0.589 \\
                        &  5 & 479 & 326 & 1.2 & 1.2 & 1.7 & 1.8 & 1.000 & 0.460 & 0.428  & 0.492 \\
                        &  20  & 1693 & 2134 & 1.6 & 10.2 & 1.9 & 2.4 & 1.000 & 0.342& 0.280& 0.337 \\
                        &  100& 1628 & 4151 & 2.5 & 12.4 & 1.2 & 2.3 & 1.000 & 0.110 & 0.144 & 0.203\\
\hline
\multirow{4}{*}{$0.01$} & 2   & 237  & 189 & 0.8 & 0.5 & 0.7 & 1.7 & 1.000 & 0.612  & 0.620  & 0.570 \\
& 5                           & 140 & 413 & 1.3 & 1.2 & 0.7  & 2.0 & 1.000 & 0.430  & 0.304  & 0.438  \\
& 20                          & 217 & 3223& 1.4 & 13.5 & 1.6 & 2.2& 1.000 & 0.267  & 0.271  & 0.245 \\
& 100                         & 544 & 5754 & 1.5 & 14.4 & 1.9 & 2.4 & 1.000 & 0.091  & 0.125  & 0.181 \\
\bottomrule
\end{tabular}
\end{small}
\end{table*}

\subsection{Simulation Environment and Metrics}
For different configurations of $(\delta, K, \Delta_1)$ for BAI, we generate 1000 independent problem instances $(\mu_i)_{i=1}^K$ by sampling each $\mu_i \in N(0,1)$ and then reset $\mu_*$ to meet the given value of $\Delta_1$. Observing that our conclusion does not vary much under different $\Delta_1$, we present the result for $\Delta_1=0.5$ in this section and leave more results in the appendix \ref{app:Delta} due to space limit. The parameters in the user model are set to $\alpha=1, \rho_t = 1+\frac{n(t)}{t} \in [1,2]$, i.e., $\rho_0=1, \rho_1=2$, and results for different choice of $\alpha$ can be found in Appendix \ref{app:additional_alpha}. We run BAIR with $N_1=\frac{2K}{\delta}$ and compare its performance with UNI, EXP3 and T\&S on the entire set of problem instances and calculate the following three metrics.
\noindent\textbf{Probability of success:} When each algorithm terminates, we examine whether the output arm is the best arm (i.e., success). The probability of success ($p$) is then given by the empirical frequency of success over all problem instances. We also calculate the value $\frac{1-p}{\delta}$ to measure if and how much the probability of success falls below the given confidence level $\delta$, which is presented right after the probability of success. \textbf{Rejection rate:} When each algorithm terminates at step $T$, we count the total number of rejections $\# Rej$ the system receives. The rejection ratio is given by $\frac{\# Rej}{T}$, and then averaged over all problem instances. \textbf{Stopping time:} It is the total number of interactions needed to terminate an algorithm. BAIR and T\&S stop by their own termination rules; UNI and EXP3 stop by the input time  $T$, since these two algorithms terminate by a preset time horizon. To make a fair comparison, we set $T$ for UNI/EXP3 as the average stopping time of BAIR under the corresponding problem instance. Hence, this metric is only set to compare BAIR and T\&S. 


\subsection{Experiment Results}



% \begin{figure*}[h]
% \centering
% \subfigure[$\Delta_1=0.5$]{
% \label{fig:subfig:a}
% \includegraphics[width=1.0\textwidth]{figure/d5.png}}
% % \hspace{.2in}
% \subfigure[$\Delta_1=0.2$]{
% \label{fig:subfig:b}
% \includegraphics[width=1.0\textwidth]{figure/d2.png}}
% % \vspace{-3mm}
% \caption{The comparison between BAIR/T\&S/EXP3/UNI for different $(\delta, K, \Delta_1)$. 
% }
% \label{fig:comparison} 
% % \vspace{-3mm}
% \end{figure*}
The results are reported in Table \ref{tb:exper-baselines}. Based on the comparison results for BAIR and the baselines, we have the following observations.  

\noindent\textbf{BAIR vs. T\&S.} As shown in Table \ref{tb:exper-baselines}, T\&S enjoys the best performance among three baselines on rejection rate and probability of success, but still does not work well in our problem setting. Given the confidence threshold $\delta$, T\&S fails to identify the best arm with probability $1-\delta$ for $K>2$ and $\delta<0.05$. We also find the stopping time of T\&S is worse than BAIR in most cases and fails to meet its theoretical lower bound $O(\log \frac{1}{\delta})$. This is expected: our binary user feedback cannot be simply modeled as independent and stationary rewards, which are the fundamental assumptions behind the design of T\&S. Since T\&S wrongly models user responses, it is easily misinformed by the user's potentially inaccurate feedback in the early stage. As a result, it is very likely to miss the best arm and spend most of the rest time on a wrong subset. In contrast to T\&S, BAIR is aware that the revealed preferences from the early stage are very likely to have a large variance. Therefore, it chooses to make safe recommendations at first to help the user gain more experiences (Phase-1 preparation) such that that the user will reveal more accurate feedback later on (Phase-2 elimination). This explains how BAIR achieves the goal more efficiently, even with the additional cost in Phase-1. 

\noindent\textbf{BAIR vs. UNI/EXP3.} The other two baselines, UNI and EXP3, exhibit worse performance in both the rejection ratio and the probability of success than BAIR. 
    % From Table \ref{tb:exper-baselines} we observe that the performance gap becomes larger when $\Delta_1$ is small, which indicates that BAIR is more competitive when facing more difficult problem instances. 
    Given the same time budget, UNI always suffers from the largest proportion of rejections because it does not take any measures to eliminate bad arms. As rejections do not update the user's empirical reward estimation, the given time budget is insufficient for UNI to differentiate the arms with similar expected rewards, thus causing a low probability of success. EXP3 enjoys a lower rejection rate than UNI, because it pulls those empirically bad arms less. The mandatory exploration in EXP3 helps correct the inaccurate early observations and gives a more competitive probability of success when $K$ gets larger. However, due to the larger variance of EXP3, if the user's estimated reward for the best arm is low at the beginning, EXP3 tends to overly focus on differentiating a group of suboptimal arms, which decreases its chance of discovering the best arm.

To summarize, the fundamental reason for the failure of these baselines lies in the insufficient system exploration when facing an explorative user. These baselines either treat the user as a black-box or assume independent and stationary user feedback, which leads to a worse empirical result in terms of both accuracy and efficiency in finding the best arm. %BAIR, however, well handles the challenge in learning from the revealed preferences by employing a more realistic user model. 

The result in Table \ref{tb:exper-baselines} supports our theoretical analysis in Theorem \ref{thm:upperbound2}. When $\Delta_1=0.5$ and $\delta<0.1$, $\frac{1}{\delta}$ dominates $\frac{1}{\Delta_1^2}$ and Theorem \ref{thm:upperbound2} suggests the algorithm's stopping time grows approximately linear in $\frac{1}{\delta}$. As expected, the first column in Table \ref{tb:exper-baselines} confirmed our theory. The first column in Table \ref{tb:exper-baselines} also suggests an approximately linear dependency between BAIR's stopping time and $K$. Although it is not fully supported by our theory (the leading term in the upper bound result is $O(K^{1.5})$ when $\alpha=1$), we believe this observation is informative and could be an interesting target for future work. 
% Since $O(K)$ is the obvious lower bound for the stopping time of BAI with fixed confidence, we may claim that BAIR's stopping time is provably optimal in $\delta$ and empirically optimal in $K$.
% that the stopping time grows linear in $\frac{1}{\delta}$ and the number of rejections is dominated by the number of acceptances when $K<\frac{1}{\delta}$. 
\subsection{Additional Experiments on the Robustness}\label{subsec:robust}
In practice, it might be too restrictive to assume that the user strictly follows our proposed confidence interval (CI) based behavior model. Thus, it is interesting and also crucial to test the robustness of BAIR under the situation where the user's behavior might deviate from the CI-based model. To this end, we extended the user model to a stochastic setting by incorporating ``decision randomness''. Specifically, we assume at each time step, with some constant probability $p$, the user makes a random decision (accept/reject the recommendation with an equal probability); otherwise, she would follow the CI-based behavior model. We demonstrate that a minor modification of BAIR still maintains competitive empirical performance in this new environment, against the three baselines. Due to space limit, we leave the detailed discussion in Section \ref{app:robust} in the appendix. 

% \begin{itemize}[leftmargin=*]
    
%     \item \textbf{The optimal choice of $N_1$.} 
%     % \item \textbf{How Phase-1 contributes to Phase-2 in BAIR.} 
%     % Although the choice of $N_1=\frac{2K}{\delta}$ seems like a squander in Phase-1, it does not affect the overall performance that much simply because a longer Phase-1 leads to a shorter Phase-2. As indicated by Table \ref{tb:exper-N1}, if we compare the stopping time of Phase-2 for $N_1=\frac{2K}{\delta}$, we will find that the system spends nearly negligible time in Phase-2 compared to Phase-1 for $\delta=0.01$. The reason is that given a large $N_1$, the system has already efficiently explored all the arms during Phase-1. As a result, when it enters Phase-2, most arms have been pulled sufficiently many times and the final eliminations can thus be executed quickly. 
% \end{itemize}

% \begin{table}[t]
% \caption{Stopping Time Comparison between BAIR and T\&S}
% \label{tb:exper-baselines}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ll|cc|cc}
% \toprule
%  &   & \multicolumn{2}{c}{$\Delta_1=0.5$} & \multicolumn{2}{c}{$\Delta_1=0.2$} \\
% $\delta$ & $K$ & BAIR & T\&S& BAIR & T\&S  \\
% \midrule
% \multirow{5}{*}{$0.1$} & 2    & 405  & 539 & 3116 & 4516 \\
% & 5                           & 737  & 1069 & 4477 & 9160 \\
% & 20                          & 2113 & 3107 & 9625 & 23600\\
% & 100                         & 10449 & 16523 & 36613 & 57596\\
% \hline
% \multirow{5}{*}{$0.05$} & 2  & 413 & 557 & 3188 & 4555 \\
%                         &  5 & 787 & 1123& 4835 & 11766 \\
%                         &  20 & 2421 & 3161& 9787  & 24283\\
%                         &  100 & 10826 & 16577 & 39415 & 60029 \\
% \hline
% \multirow{5}{*}{$0.02$} & 2  & 422 & 544& 3202 & 4602 \\
%                         &  5 & 879 & 1148 & 4885 & 12037 \\
%                         &  20 & 3593 & 3210 & 9881 & 26799\\
%                         &  100 & 11528 & 16955& 40626 & 66454 \\
% \hline
% \multirow{5}{*}{$0.01$} & 2   & 437  & 554  & 3384 & 4623\\
% & 5                           & 940 & 1153 & 4921 & 13601\\
% & 20                          & 4017 & 3223 & 10050 & 26952\\
% & 100                         & 20344& 27548 & 41885 & 69039\\
% \hline
% \multirow{5}{*}{$0.005$} & 2   & 512 & 570 & 3426 & 4683\\
% & 5                            & 1692 & 1580 & 5022 & 16024\\
% & 20                           & 7827 & 5983 & 10544 & 30502\\
% & 100                         & 40246 & 37931& 43868 & 82005 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}




==> macro.tex <==

 \newcommand{\todo}[1]{{\color{red}\noindent[ToDos: #1]}}
% \newcommand{\linit}{\ell_{init}}
% \newcommand{\hf}[1]{{\color{blue}  [\text{Haifeng:} #1]}}
% \newcommand{\fan}[1]{{\color{green}  [\text{Fan:} #1]}}
% \newcommand{\anil}[1]{{\color{red}  [\text{anil:} #1]}}

\newcommand{\linit}{\ell_{init}}
\newcommand{\fan}[1]{\textcolor{blue}{#1}}
\newcommand{\anil}[1]{\textcolor{red}{#1}}


\newenvironment{proofof}[1]{\begin{proof}[Proof of #1]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[Proof Sketch]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[Proof Sketch of #1]}{\end{proof}}


%regular version
\def\pr{\qopname\relax n{Pr}}
\def\ex{\qopname\relax n{E}}
\def\min{\qopname\relax n{min}}
\def\max2{\qopname\relax n{max2}}
\def\max{\qopname\relax n{max}}
\def\argmin{\qopname\relax n{argmin}}
\def\argmax{\qopname\relax n{argmax}}
\def\avg{\qopname\relax n{avg}}


%bold version
\def\Pr{\qopname\relax n{\mathbf{Pr}}}
\def\Ex{\qopname\relax n{\mathbf{E}}}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\II}{\mathbb{I}}

\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\P{\mathcal{P}}
\def\R{\mathcal{R}}
\def\S{\mathcal{S}}
\def\O{\mathcal{O}}
\def\T{\mathcal{T}}
\def\V{\mathcal{V}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}

\def\eps{\epsilon}

\def \cD {\mathcal{D}}
\def \cG {\mathcal{G}}
\def \cH {\mathcal{H}}
\def \cR {R}
\def \cX {\mathcal{X}}
\def \cY {\mathcal{Y}}

%%% Vectors 
\def\x{\bm{x}} 
\def\XX{\textbf{X}} 
\def\y{\bm{y}} 
\def\w{\bm{w}} 
\def\c{\bm{c}} 
\def\e{\bm{e}} 
\def\r{\bm{r}} 
\def\v{\bm{v}} 
\def\z{\bm{z}} 
\def\p{\bm{p}} 
\def\q{\bm{q}} 
\def\u{\bm{u}} 
\def\v{\bm{v}} 




%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
\newcommand{\maxis}[1]{\mbox{max} & {#1 } & \\}
\newcommand{\minis}[1]{\mbox{min} & {#1 } & \\}
\newcommand{\find}[1]{\mbox{find} & {#1 } & \\}
\newcommand{\stt}{\mbox{subject to} }
\newcommand{\sts}{\mbox{s.t.} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation} }
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}

%misc
\newcommand{\probdet}{\textsc{StraC}}
\newcommand{\prob}{\textsc{StraC}$\langle \cH, R, c  \rangle$} 
\newcommand{\probL}{\textsc{StraC}$\langle \cH_d, R, c  \rangle$} 
\newcommand{\probrand}{\textsc{RandSC}}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}





==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\standarderror}{\mathrm{SE}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\let\ab\allowbreak


==> model.tex <==
\section{Modeling Users' Revealed Preferences}\label{sec:model}

%In this section, we first present the problem setting on both the user side and the system side, and then describe our user behavior model, which constitutes the basis for learning from explorative users' revealed preferences. 

%\subsection{Problem Formulation}
To study the sequential interactions between a recommender system and an explorative user, we adopt a stochastic bandit framework where the time step $t$ is used to index each interaction, and the set of arms $[K]=\{1,\cdots,K\}$ denote the recommendation candidates. At each time step $t$, the following events happen in order:
\begin{enumerate}
    \item The system recommends an arm $a_t$ to the user;
    \item The user decides whether to accept or reject $a_t$. If the user accepts $a_t$, realized reward $r_{a_t, t}$ is disclosed to the user afterwards.
    \item The system observes the user's binary   decision of acceptance or not, i.e., the   revealed preference \cite{richter1966revealed}.  
\end{enumerate}

From the user's perspective, we denote the true reward of each arm $i \in [K]$ as $\mu_i$, and the realized reward after each acceptance of arm $i$ is drawn independently from a sub-Gaussian distribution with mean $\mu_i$ and unit variance. 
%We postpone the details about how the user responds to the system's recommendation in the next subsection.   %We can further assume that the sequence of rewards for each arm is drawn before the interaction starts, so that the empirical reward for arm $i$ at each time step $t$ is well defined as an i.i.d. sequence $\{r_{i,t}\}_{t=1}^{\infty}$ drawn from the reward distribution even if $i$ has not been actually recommended or accepted at step $t$. 
% The item pool is represented by a set of $K$ arms, denoted by $[K]=\{1,\cdots,K\}$. We may view each arm a single item or a category of items and parameterized by its expected payoff $\mu_i$. At each time step $t$, the system recommends an arm $i\in [K]$ to the user, and the user may choose to accept or decline the recommendation. If the user accepts, she will observe a reward $r_{i,t}\sim N(\mu_i, 1)$ drawn from a Gaussian distribution with mean $\mu_i$ and unit variance; if the user rejects, she will not receive any feedback from the item and thus maintains the same empirical mean estimation for each arm. In addition, we assume the realized rewards are only kept by the user, meaning the system can only observe the user's binary decision from each interaction. 
The system has a long-term objective and aims to find the best arm while minimizing the total number of recommendations. This renders our problem   a best arm identification (BAI) problem with fixed confidence but based on partial information about the rewards.
%, as the system cannot observe the payoff behind each pull. %We will discuss how the system can still infer the best arm efficiently under a reasonable user behavior model. 
Throughout the paper, we assume without loss of generality that $\mu_*=\mu_1>\mu_2\geq \mu_3\geq \cdots \geq \mu_K$, and let $\Delta_1=\mu_1-\mu_2, \Delta_i = \mu_{*} - \mu_i > 0, \forall i >1.$ Following the convention in BAI literature \cite{carpentier2016tight,audibert2010best}, we further define the quantity $H=\sum_{i=1}^K \frac{1}{\Delta_i^2}$ which characterizes the hardness of the problem instance. 

%\subsection{User Behavior Modeling}\label{sec:usermodel}
As discussed previously, the user cannot choose from the full arm set but can only decide whether to accept or reject the recommended arms from the system. To make a decision at time $t$, we assume the user utilizes the information in all previous interactions by maintaining a confidence interval $CI_{i,t}=(lcb_{i,t},ucb_{i,t})$ for each arm $i$, which is defined as 
\begin{equation*}
    (lcb_{i,t},ucb_{i,t})\triangleq\left(\hat{\mu}_{i,t}-\sqrt{\frac{\Gamma(t;\rho,\alpha)}{n_i^t}},\hat{\mu}_{i,t}+\sqrt{\frac{\Gamma(t;\rho,\alpha)}{n_i^t}}\right),
\end{equation*} 
where $lcb$ and $ucb$ stand for the lower/upper confidence bounds respectively, $n_i^t$ is the number of 
\emph{acceptances} on arm-$i$ up to time $t$, $\hat{\mu}_{i,t}=\frac{1}{n_i^t}\sum_{s=1}^t \mathbb{I}[i \text{~is~accepted~at~} s]r_{i,s}$ is the empirical mean reward of arm $i$ at time $t$, and $\Gamma(t;\rho,\alpha)$ is a function parameterized by $\{\rho_t,\alpha\}$, which characterize the user's confidence level to her reward estimation at time step $t$. 
% A larger value of $\Gamma$ implies a higher user's tolerance for the current recommendation, and thus a stronger inclination to explore. 
Following the convention rooted in the UCB1 algorithm \cite{auer2002finite}, we consider the (flexible) confidence bound form:
\begin{equation}\label{eq:trust}
    \Gamma(t;\rho,\alpha)=\max\left\{0, 2\alpha\log [\rho_t \cdot n(t)]\right\},
\end{equation}
where $n(t)=\sum_{i\in [K]}n_i^t$ is the total number of accepted recommendations up to time $t$. We note that the choice of $\Gamma$ is to   flexibly cover possibly varied user types  captured by parameters $\alpha$ and $\rho_t$. In particular, $\alpha$ directly controls the span of the CIs and thus represents the user's intrinsic tendency to explore: a larger $\alpha$ indicates a higher tolerance for the past observations, meaning the user is more willing to accept recommendations in a wider range. $\rho_t: \mathbb{N} \xrightarrow{} [\rho_0, \rho_1]$ is allowed to be any sequence that can depend on the interaction history and has a bounded range $[\rho_0, \rho_1] \subset (0, +\infty)$, which captures the cases where the user's confidence over the system evolves over time. For example, $\rho_t$ can be a function of the acceptance rate $\frac{n(t)}{t} \in [0, 1]$ and increases monotonically with respect to $\frac{n(t)}{t}$. Our results only rely on the lower and upper bound of $\rho_t$ and are oblivious to its specific format. Note that for the special case of $\alpha=1, \rho_t=1 \,  \forall t$, Eq \eqref{eq:trust} corresponds to 
%the case when the user makes acceptance or rejections depending on 
the classic confidence interval defined in UCB1. We remark that parameters $\alpha$ and $\rho_t$ are     only to characterize different types of users, which provide flexibility in handling different real-world scenarios; but they are \emph{not} introduced for our solution.
%, except that she does not has the freedom to pull an arbitrary arm but only the recommended one. 
% We note that our choice of $\rho_t$ is general enough to accommodate a wide range of user behavior, and the theoretical analysis only requires $\rho_t$ to have a bounded range. We also point out the choice of $\alpha$ does not essentially affect our main result in spirit. Therefore, for simplicity purpose we consider the case $\alpha=1$ through out the paper without loss of generality and omit $\rho$ in the expression of $\Gamma$ if it does not cause any confusion hereinafter.

\noindent
\textbf{The decision rule.} %Next, we discuss user's decision rule when facing a recommendation. 
When an arm $i$ is recommended, we assume the user will reject it if and only if   there exists $j \neq i$ such that $lcb_j \geq ucb_i$. That is, the user only accepts an arm if  there is no other arm that is clearly better than the recommended one with a high confidence. 
%Formally,  the acceptance rule can be stated as follows: the user will accept arm $i$ either when $i$ is the one with the highest $lcb$ (denoted by $a_t^*$) or $CI_{i,t} \cap CI_{a_t^*,t} \neq \varnothing$. 
The rationale behind our imposed user decision rule is straightforward: first, the user should not miss the arm with the highest lower confidence bound as this is arguably the safest choice for the user at the moment; second, if two arms have chained confidence intervals, the user does not have enough information to distinguish which one is better, and hence should not reject either one, i.e., being explorative. 
% \begin{enumerate}
%     \item $I_t$ is the one with the highest lower confidence bound, i.e., $I_t = I_t^* \triangleq \arg\max_{i\in [K]} lcb_{i,t}$.
%     \item The confidence interval of $I_t$ overlaps with the confidence interval of $I_t^*$.
% \end{enumerate}

% We define two types of users accordingly. The type-1 user can only apply the second rule once, meaning the she would only accept those arms whose confidence intervals overlaps with $CI_{\hat{I}_t^*,t}$. The type-2 user may apply the second rule recursively so that any arm whose confidence interval is chained 
% with $CI_{\hat{I}_t^*,t}$ will be accepted. Clearly, the type-2 user is more inclined to explore sub-optimal choices compared to type-1 user. We analyze the system's learning strategy when facing both type-1 and type-2 users and will show later there is only minor differences.



% Note that if the user is allowed to apply the second rule recursively, i.e., also accepts those arms whose confidence intervals are chained with $I_t^*$, the behavior pattern coincides with the setting discussed in the fairness bandit problem \cite{joseph2016fairness}. In fairness bandit, the system has to pull any pair of arm with overlapping confidence intervals with equal probability to guarantee fairness. Our model does not emphasis the fairness issue but aims to capture the behavior of a reasonably myopic user: she would always prefer the arm with the best historical performance, but is also willing to try sub-optimal arms as long as she is not confident enough to reject them based on her trust to the system.
